From Abstract to Contextual: What LLMs Still Cannot Do in Mathematics

Large language models now solve many benchmark math problems at near-expert levels, yet this progress has not fully translated into reliable performance in real-world applications. We study this gap through contextual mathematical reasoning, where the mathematical core must be formulated from descriptive scenarios. We introduce ContextMATH, a benchmark that repurposes AIME and MATH-500 problems into two contextual settings: Scenario Grounding (SG), which embeds abstract problems into realistic narratives without increasing reasoning complexity, and Complexity Scaling (CS), which transforms explicit conditions into sub-problems to capture how constraints often appear in practice. Evaluating 61 proprietary and open-source models, we observe sharp drops: on average, open-source models decline by 13 and 34 points on SG and CS, while proprietary models drop by 13 and 20. Error analysis shows that errors are dominated by incorrect problem formulation, with formulation accuracy declining as original problem difficulty increases. Correct formulation emerges as a prerequisite for success, and its sufficiency improves with model scale, indicating that larger models advance in both understanding and reasoning. Nevertheless, formulation and reasoning remain two complementary bottlenecks that limit contextual mathematical problem solving. Finally, we find that fine-tuning with scenario data improves performance, whereas formulation-only training is ineffective. However, performance gaps are only partially alleviated, highlighting contextual mathematical reasoning as a central unsolved challenge for LLMs.

==> dkvyckmztzhccsnhttrnhthhdxwytnqw/Ethics_statement.tex <==
\section*{Ethics Statement}
This work studies LLMs through the lens of contextual mathematical reasoning. 
All data used are derived from publicly available math benchmarks (AIME and MATH‑500), with additional scenario variants generated automatically and verified for mathematical equivalence. 
No private or sensitive data were used. 
We evaluate only open‑source and commercially available models, and all experiments are conducted under non‑interactive settings without user data collection. 
While our results reveal limitations of current LLMs, these findings are intended to encourage more rigorous evaluation and robust model design, not to promote unsafe deployment. 
We will release our benchmark openly to facilitate reproducibility and further research, subject to the same usage terms as the underlying datasets. 

==> dkvyckmztzhccsnhttrnhthhdxwytnqw/Reproducibility_statement.tex <==
\section*{Reproducibility Statement}
We take reproducibility seriously in this work. The construction pipeline of \textbf{ContextMATH}, including all generation, verification, and revision prompts, is detailed in Section~\ref{benchmark} and Appendix~\ref{appx:instruction}. Evaluation setups are described in Appendix~\ref{app:evaluation_details}, with complete accuracy results for open‑source models reported in Appendix~\ref{app:opensource_results}, and results for proprietary models in Table~\ref{tab:proprietary_model_performance}. The analysis of formulation metrics is presented in Section~\ref{analysis}, with full breakdowns in Appendix~\ref{appx:formulation_results}. Implementation details of all training experiments are provided in Appendix~\ref{implementation details}. We will release our benchmark publicly, ensuring that independent researchers can fully reproduce our benchmark, analyses, and training results.

==> dkvyckmztzhccsnhttrnhthhdxwytnqw/SFT_results.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{l ccc ccc cc cc c S[table-format=2.1]@{\hspace{1pt}}c}
% \begin{tabular}{lc*{12}{p{0.6cm}}}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{AIME 2024 (\%)}} & \multicolumn{3}{c}{\textbf{AIME 2025 (\%)}} & \multicolumn{2}{c}{\textbf{Math (\%)}}  & \multicolumn{2}{c}{\textbf{Math-P (\%)}} & \multirow{2}{*}{\textbf{AMC23}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Average}}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
& \multicolumn{1}{c}{\textbf{Ori}} & \multicolumn{1}{c}{\textbf{SG}} & \multicolumn{1}{c}{\textbf{CS}} & \multicolumn{1}{c}{\textbf{Ori}} & \multicolumn{1}{c}{\textbf{SG}} & \multicolumn{1}{c}{\textbf{CS}} & \multicolumn{1}{c}{\textbf{Ori}} & \multicolumn{1}{c}{\textbf{SG}} & \textbf{Simple} & \textbf{Hard} \\
\midrule
Qwen3-4B-Base & 9.8 & 6.2 & 3.3 & 8.1 & 4.0 & 0.8 & 51.7 & 40.3 & 53.5 & 34.6 & 43.4 & 23.3 & (+\ \ 0.0\%) \\
+ $\text{SFT}_{\text{Ori.}}$ & 32.5 & 27.3 & 14.2 & 27.9 & 18.5 & 11.5 & 80.5 & 65.5 & 81.2 & 66.3 & 75.6 & 45.6 & (+22.3\%) \\
+ $\text{SFT}_{\text{Syn.}}$ & 34.2 & \best{32.1} & 17.3 & \best{31.7} & 20.2 & 11.9 & 78.8 & 70.8 & 80.0 & 65.1 & 74.7 & 47.0 & (+23.7\%) \\
+ $\text{SFT}_{\text{Mix}}$ & \best{36.9} & 31.7 & \best{19.2} & 30.2 & \best{22.1} & \best{12.7} & \best{81.4} & \best{72.3} & \best{82.7} & \best{69.0} & \best{78.1} & \best{48.8} & (+\best{25.5}\%) \\
\midrule
Qwen3-8B-Base & 13.3 & 7.5 & 2.9 & 10.2 & 6.0 & 1.2 & 58.5 & 46.2 & 61.1 & 38.9 & 54.4 & 27.3 & (+\ \ 0.0\%) \\
+ $\text{SFT}_{\text{Ori.}}$ & 44.4 & 35.4 & 20.0 & 32.7 & 21.2 & 15.0 & 85.7 & 74.0 & \best{86.9} & 73.6 & 83.9 & 52.1 & (+24.8\%) \\
+ $\text{SFT}_{\text{Syn.}}$ & \best{47.7} & \best{44.8} & \best{30.6} & \best{37.5} & 25.8 & \best{20.6} & 84.4 & 76.4 & 85.6 & 72.8 & 83.3 & 55.4 & (+27.9\%) \\
+ $\text{SFT}_{\text{Mix}}$ & 46.2 & 42.4 & 29.5 & 35.9 & \best{26.8} & 20.5 & \best{85.9} & \best{76.7} & \best{86.9} & \best{74.4} & \best{86.6} & \best{55.6} & (+\best{28.3}\%) \\
\midrule
Qwen3-14B-Base & 14.8 & 11.0 & 4.8 & 10.2 & 7.1 & 1.2 & 60.8 & 50.2 & 63.5 & 43.9 & 55.9 & 29.4 & (+\ \ 0.0\%) \\
+ $\text{SFT}_{\text{Ori.}}$ & 50.4 & 39.0 & 25.2 & 41.7 & 25.2 & 20.4 & 85.9 & 73.4 & 85.5 & 75.0 & 89.1 & 55.5 & (+26.1\%) \\
+ $\text{SFT}_{\text{Syn.}}$ & \best{58.3} & 46.4 & \best{38.8} & \best{50.0} & 30.3 & 23.9 & 85.5 & 77.5 & \best{88.7} & \best{76.3} & 88.9 & 60.4 & (+31.0\%) \\
+ $\text{SFT}_{\text{Mix}}$ & 56.5 & \best{52.5} & \best{38.8} & 47.2 & \best{34.6} & \best{26.5} & \best{86.7} & \best{77.8} & 88.2 & 76.1 & \best{89.8} & \best{61.3} & (+\best{31.9}\%) \\
\bottomrule
\end{tabular}
\caption{
Performance of \texttt{Qwen3-Base} models after supervised fine-tuning. Each base model is compared with variants trained on original problems (SFT$_{\text{Ori}}$), synthetic scenario problems (SFT$_{\text{Syn}}$), or their mixture (SFT$_{\text{Mix}}$). The best result within each block is highlighted in \textbf{bold}.}
\label{tab:sft_main_results}
\end{table}


==> dkvyckmztzhccsnhttrnhthhdxwytnqw/abstract.tex <==
\begin{abstract}
Large language models now solve many benchmark math problems at near‑expert levels, yet this progress has not fully translated into reliable performance in real‑world applications. 
We study this gap through \textit{contextual mathematical reasoning}, where the mathematical core must be formulated from descriptive scenarios.
We introduce \textbf{ContextMATH}, a benchmark that repurposes AIME and MATH-500 problems into two contextual settings: Scenario Grounding (SG), which embeds abstract problems into realistic narratives without increasing reasoning complexity, and Complexity Scaling (CS), which transforms explicit conditions into sub‑problems to capture how constraints often appear in practice. 
Evaluating 61 proprietary and open‑source models, we observe sharp drops: on average, open‑source models decline by 13 and 34 points on SG and CS, while proprietary models drop by 13 and 20.  
Error analysis shows that errors are dominated by incorrect problem formulation, with formulation accuracy declining as original problem difficulty increases. Correct formulation emerges as a prerequisite for success, and its sufficiency improves with model scale, indicating that larger models advance in both understanding and reasoning. Nevertheless, formulation and reasoning remain two complementary bottlenecks that limit contextual mathematical problem solving. Finally, we find that fine‑tuning with scenario data improves performance, whereas formulation‑only training is ineffective. 
However, performance gaps are only partially alleviated, highlighting contextual mathematical reasoning as a central unsolved challenge for LLMs.
\end{abstract}




==> dkvyckmztzhccsnhttrnhthhdxwytnqw/ack.tex <==
\section*{Acknowledgement}
The work described in this paper is substantially supported by a grant from the Direct Grant of Faculty of Engineering, The Chinese University of Hong Kong (Project Code: 4055275).

==> dkvyckmztzhccsnhttrnhthhdxwytnqw/analysis.tex <==
\section{Analysis of Failure Modes: The Formulation Bottleneck}
\label{analysis}
The performance degradation observed in Section \ref{benchmark} motivates an analysis of the underlying failure modes. Our central hypothesis is that these failures do not primarily stem from flawed computational reasoning, but from the incorrect interpretation of the problem's mathematical structure from its narrative context. This section validates this hypothesis through a combination of qualitative analysis and quantitative experiments that isolate contextual mathematical problem formulation skill.

% \vspace{-1mm}
\subsection{Qualitative Analysis: Incorrect Mathematical Interpretation}
 
To examine how such failures occur, we ask \texttt{GPT‑5} to categorize the errors made by \texttt{DeepSeek R1}, \texttt{Gemini 2.5 Pro}, and \texttt{Qwen3‑32B} on the SG and CS sets of AIME 2024 and 2025, restricted to cases where the same models solve the original version correctly. 

\begin{wrapfigure}{h}{0.51\textwidth}
\vspace{-4mm}
\centering
\includegraphics[width=\linewidth]{error_count.pdf} 
\caption{
Distribution of error types in failure cases on AIME 2024/2025 SG and CS problems, where ratios indicate the proportion of cases exhibiting each error type.
}
\label{Fig.error_count}
\end{wrapfigure}
Errors are grouped into four categories: formulation (incorrect mapping from narrative to math), calculation, logic, and other (e.g., truncation, repetition). 
Figure~\ref{Fig.error_count} shows that formulation errors dominate, accounting for roughly 80\% of failures across all three models and far exceeding any other type. 
A typical case is given in Appendix~\ref{appx:R1_example}, where \texttt{DeepSeek R1} fails to recognize that “\textit{the time for a gear to complete one rotation is adjustable, but it must not exceed six rotations per minute}” implies the inequality $x \geq 10$, with $x$ denoting seconds per rotation. This consistent pattern confirms that formulation is the primary weakness in contextual reasoning.
This presents an interesting contrast with \cite{cheng-etal-2025-llms}: while their findings suggest that abstract formulation is not the primary bottleneck on simpler benchmarks like GSM8K \citep{cobbe2021gsm8k}, our work demonstrates that formulation becomes a critical bottleneck once the mathematical core is embedded in complex, contextual narratives.

\input{quantitative_merged}

% \vspace{-1mm}
\subsection{Quantitative Validation: Evaluating Problem Formulation from Context}
\label{sec:quantitative}
In this section, we evaluate a model’s ability to abstract a mathematical formulation from a given scenario.
For each problem in the SG and CS test sets, the model is prompted to output only the core formulation, stripped of all narrative details.
In addition to reporting formulation accuracy, we analyze the necessity and sufficiency of correct formulations for correct reasoning, highlighting the fundamental relationship between them.

% \vspace{-2mm}
\paragraph{Evaluation Setups.}
We carefully design the instructions and examples to prompt \texttt{o1‑mini} as an automated judger, which determines whether the model’s output is mathematically equivalent to the original problem.\footnote{We manually annotated the outputs of \texttt{Qwen3‑14B} and \texttt{Qwen3‑32B} and found that the judger’s assessments align with human judgments in over 90\% of cases.}
For each problem, we evaluate 16 samples using the same seed set as in our benchmark evaluation (Section~\ref{benchmark}) and report three complementary metrics.
The first is \colorbox{lightyellow!50}{Formulation Accuracy}, defined as the mean of the judger’s assessments across samples.  
The second is Formulation Necessity, which measures how often a correct problem formulation is required for a correct solution. Formally, let $F$ denote whether the formulation is correct and $R$ whether the reasoning produces the correct answer. Necessity is defined as the conditional probability 
\begin{equation}
\vspace{-0.5mm}
    \colorbox{MintGreen!50}{\text{Formulation Necessity}} = P(F=\text{True} \mid R=\text{True}) .
\vspace{-0.5mm}
\end{equation}
This quantifies the consistency of the relation $R \!\Rightarrow\! F$.  
The third is Formulation Sufficiency, which evaluates whether a correct formulation reliably leads to a correct solution. It is given by  
\begin{equation}
\vspace{-0.5mm}
\colorbox{BabyBlue!50}{\text{Formulation Sufficiency}} = P(R=\text{True} \mid F=\text{True}) .
\vspace{-0.5mm}
\end{equation}
This corresponds to the coverage of the relation $F \!\Rightarrow\! R$.  
Together, these three metrics offer a coherent perspective: accuracy captures overall performance, while necessity and sufficiency jointly characterize the directional dependency between formulation and reasoning.

\begin{wrapfigure}{h}{0.51\textwidth}
\vspace{-5mm}
\centering
\includegraphics[width=\linewidth]{pattern_analysis.pdf} 
\caption{
% Relationship between reasoning accuracy and formulation metrics. Each point represents a model, with the x-axis showing its average reasoning accuracy across all subsets. The fitted lines indicate the overall trends.
Relationship between reasoning accuracy and formulation metrics. Each point represents a model, with the x-axis showing its average reasoning accuracy across all subsets and the y-axis showing the corresponding values of formulation accuracy (orange), necessity (green), and sufficiency (blue). The fitted lines indicate the overall trends.
}
\label{Fig.analysis}
\end{wrapfigure}

% \vspace{-2mm}
\paragraph{Results.}
To present an overview of model behavior, we report aggregated formulation metrics in Table~\ref{tab:formulation_results}, where the AIME24 and AIME25 scores are averaged over their SG and CS sets for simplicity, while the full breakdown is provided in Appendix~\ref{sec:formulation_full}. To further analyze the relationship between formulation and overall task performance, we also combine these metrics with the reasoning accuracies from Section~\ref{benchmark} and visualize the correlations in Figure~\ref{Fig.analysis}. Our findings can be summarized into three key insights:

\textbf{(i) Formulation accuracy declines with problem difficulty.} 
Table~\ref{tab:formulation_results} shows that formulation accuracy (orange) decreases steadily from MATH-500 to AIME24 to AIME25 (e.g., \texttt{Qwen3‑4B}: 84.8\% $\to$ 64.6\% $\to$ 47.1\%), consistent with the increasing difficulty of the underlying problems. 
This trend shows that problems with a harder mathematical core remain more difficult for models to formulate correctly.
Scaling improves performance (e.g., \texttt{Qwen3‑0.6B} averages 42.8\% vs. 75.0\% for \texttt{Qwen3‑32B}), but even \texttt{GPT‑5} remains below 75\% on AIME25, underscoring that the formulation challenge grows with problem difficulty and cannot be resolved by scale alone.

\textbf{(ii) Correct formulation is highly necessary for correct reasoning.} On average, necessity (green) is consistently above accuracy across all models. For example, \texttt{Qwen3‑4B} achieves 61.6\% accuracy vs. 79.2\% necessity, and \texttt{GPT‑5} 81.4\% vs. 85.6\%. Figure~\ref{Fig.analysis} confirms this pattern: necessity closely tracks reasoning accuracy but is consistently higher, indicating that correct reasoning greatly depends on having a correct formulation.

\textbf{(iii) Beyond formulation, reasoning ability still limits success.} Sufficiency (blue) improves with scale but lags behind both accuracy and necessity. In Table~\ref{tab:formulation_results}, \texttt{Qwen3‑8B} records 73.8\% accuracy and 83.8\% necessity but only 60.7\% sufficiency, while \texttt{GPT‑5} achieves 82.7\% sufficiency. Figure~\ref{Fig.analysis} further highlights this gap: sufficiency rises with reasoning performance but consistently trails necessity, indicating that while correct formulation is indispensable, reliably completing the reasoning process remains challenging even for the strongest models, thus forming a second bottleneck.




==> dkvyckmztzhccsnhttrnhthhdxwytnqw/benchmark.tex <==
\section{Probing LLMs’ Ability to Solve Math in Scenarios}
\label{benchmark}
\subsection{Overview}
A central question of this work is whether LLMs possess \textit{contextual mathematical reasoning}—the ability to formulate and solve the mathematical core when problems are embedded in descriptive scenarios. This capacity is crucial for applying mathematics in practical domains, where tasks rarely appear as ready‑made equations. Collecting large numbers of real‑world instances, however, is costly and difficult to scale. We therefore leverage established benchmarks with guaranteed correctness and systematically transform them into contextual variants. Concretely, we build \textbf{ContextMATH}, which instantiates each benchmark problem in two forms: \textit{Scenario Grounding}, preserving the original structure but embedding it in narrative context; and \textit{Complexity Scaling}, encoding explicit conditions into simple sub‑problems. We then evaluate a diverse set of 46 open‑source models and 15 proprietary models, including \texttt{GPT‑5} and \texttt{DeepSeek‑R1}.

\input{pro_model_results}

\input{main_results_short}

\subsection{Benchmark Construction}
Our benchmark is constructed from AIME 2024, AIME 2025, and MATH‑500\footnote{We select only problems with difficulty level $\geq\!3$ from MATH‑500, since easier items are less suitable for embedding into meaningful scenarios. For simplicity, we continue to refer to this filtered subset as MATH‑500 throughout the paper. We do not construct the CS set for MATH‑500 because some remaining items are too trivial to transform further, e.g., `Evaluate $(1 + 2i)(6 - 3i)$.`.}.
Our design follows two principles: preserving mathematical equivalence and embedding problems in realistic narrative contexts. To realize this, we employ a series of structured prompts that guide an LLM (\texttt{o1‑mini}) through iterative scenario generation, self‑verification, and revision. Human experts then review and refine each item to guarantee mathematical equivalence, clarity and conciseness\footnote{The average lengths of SG and CS problems are 133 and 176 words, respectively, both well within the processing capabilities of current LLMs.}.


\vspace{-3mm}
\paragraph{Scenario Grounding (SG): Evaluating the Application of Math in Context.}
The primary goal of scenario grounding is to assess whether a model can apply its mathematical knowledge when problems are presented in a narrative context, without increasing the core reasoning difficulty.
To achieve this, our generation process is guided by a multi-step prompt that instructs the model to first explicitly map all abstract mathematical elements to specific real-world objects (e.g., mapping \textit{"a variable x"} to "\textit{the initial number of barrels of oil}"). The prompt then directs the model to define the rules of interaction between these objects based on the attributes and relationship in the problem. This structured approach ensures that all mathematical components of the original problem are preserved in the final scenario (see Appendix \ref{appx:instruction} for the full prompt). 


\vspace{-3mm}
\paragraph{Complexity Scaling (CS): Encoding Implicit Constraints through Sub-Problems.}  
In many real-world settings, quantitative conditions must be inferred from indirect descriptions, such as simple calculations, relative positions, or everyday facts. To reflect this natural form of complexity, CS problems transform some direct conditions into the outputs of simple, self-contained sub-problems. For example, instead of stating there are \textit{"25 indicator lights"}, the problem may specify that \textit{"the total number of unique pairs of indicator lights is exactly 300"}. Our generation prompt provides principled strategies for such transformations, including encoding values as the solutions to number theory or combinatorics problems, replacing explicit functions or constants with variables to be determined from given data points, and rephrasing geometric relationships in terms of physical or structural descriptions. 
This design also provides a more faithful and robust test of a model’s reasoning ability by reducing reliance on superficial pattern matching, a behavior widely documented in prior studies showing the limited generalization of LLMs~\citep{cao2024worst,sun2025omega}.

\vspace*{-1mm}
\paragraph{Quality Control.} We place high importance on data quality. Our approach involves two key measures: first, we have optimized the instructions and generation pipeline through extensive pilot studies; second, our procedure involves three experts, all with advanced degrees in Computer Science and backgrounds in competitive mathematics, to fundamentally ensure accuracy. They conduct independent reviews based on the following criteria:
\begin{itemize}
[leftmargin=1em,labelsep=0.1em,topsep=0.em,itemsep=0.em]
    \item Assessing the scenario for narrative plausibility and clarity, ensuring it introduces no unnecessary complexity or ambiguity.
    \item Independently formulating an abstract math problem from the scenario to verify its solvability and mathematical equivalence to the original.
    \item Testing the scenario on Gemini and GPT-5; if these models fail, the reviewer diagnoses whether the failure originates from an ambiguity in the problem description.
\end{itemize}
A scenario is accepted only after passing all checks. Any identified issue flags the scenario for revision. In cases of disagreement, the reviewer with the strongest mathematical background leads a discussion to reach a consensus, which may trigger a regeneration or revision cycle.

\vspace{-1mm}
\subsection{Evaluation Setup}
\vspace{-1mm}
\paragraph{Models.}
We evaluate 46 advanced open-source models (including base, SFT, and RL-tuned) and 15 frontier proprietary models\footnote{Since AIME 2024 and AIME 2025 results already established a performance trend for proprietary models, and given the high API costs of Math-500, we excluded proprietary models from this part of the evaluation.}. Details are provided in Appendix~\ref{app:evaluation_details}.

\vspace*{-1mm}
\paragraph{Metrics.}
We use accuracy as the performance metric. For open-source models, we sample 16 solutions per problem using their recommended generation configurations and report the average accuracy. For proprietary models, which are accessed via APIs or client interfaces that often have rate limits or higher costs, we report the accuracy of a single-pass evaluation.


\vspace{-1mm}
\subsection{Results}
\label{benchmark_results}
% \vspace{-1mm}
Our main experimental results, presented in Table~\ref{tab:proprietary_model_performance} and \ref{tab:model_performance_short}, reveal three clear insights:

\vspace{-1mm}
\paragraph{Contextual Complexity as a Universal Bottleneck.}
Both open-source and proprietary models show consistent and severe performance drops on contextual scenarios. For instance, \texttt{DeepSeek-R1-0528-Qwen3-8B} falls from 75.0\% on AIME 2024 to 39.6\% on its CS variant, and \texttt{QwQ-plus} from 86.7\% to 46.7\%. Even \texttt{GPT-5}, with an estimated 1.8T parameters, drops 26\% on AIME 2025-CS. These findings make clear that contextual mathematical reasoning remains a fundamental and unresolved challenge, underscoring that progress on abstract math does not fully translate into robust performance in contextual settings.


\vspace{-1mm}
\paragraph{Scale Mitigates but Does Not Solve the Problem.}
In open-source evaluations, larger models retain more robustness, but scaling does not eliminate contextual failure. In the \texttt{OpenMath-Nemotron} series on AIME 2024-CS, the 1.5B model drops 77\%, compared to 43\% and 51\% for 14B and 32B. Similar trends hold for \texttt{R1-Distil-Qwen2.5} and \texttt{Qwen3} families. Larger models are more resilient, but interpreting complex narratives remains a core bottleneck.


\vspace{-1mm}
\paragraph{Initial SFT Improves Robustness, but Further Specialization Does Not.}
A first stage of supervised fine‑tuning consistently improves both original and contextual accuracy. For example, \texttt{Qwen2.5-Math-7B}$\rightarrow$\texttt{R1-Distil-Qwen-7B} not only boosts AIME accuracy but also reduces contextual drop. 
However, further SFT or RL for advanced reasoning does not improve contextual tasks. Models such as \texttt{R1-Distil-Qwen-7B}$\rightarrow$\texttt{AceMath-RL-Nemotron-7B} and \texttt{Qwen3-8B}$\rightarrow$\texttt{DeepSeek-R1-0528-Qwen3-8B} improve on AIME 2024/25 but not on SG or CS, often with even larger drops. This suggests current post-training can over-specialize to canonical formats, reinforcing pattern recognition rather than contextual reasoning.



==> dkvyckmztzhccsnhttrnhthhdxwytnqw/conclusion.tex <==
\section{Conclusion}
In this paper, we investigate LLMs’ ability to perform \textit{contextual mathematical reasoning}, where the mathematical core must be extracted from narrative context before solving.  
Through the ContextMATH benchmark, we shows that models which perform strongly on abstract math exhibit large drops on contextual variants, with errors dominated by problem formulation. 
Our analyses identify formulation and reasoning as two complementary bottlenecks that jointly constrain performance. Although these processes may intertwine in complex problems, our controlled framework provides a first step toward disentangling them and demonstrates that formulation constitutes a key obstacle.
We further show that end-to-end training with contextual data improves robustness, while directly training a dedicated formulation model is ineffective.  
Overall, our study establishes contextual mathematical reasoning as a central unsolved capability of LLMs and highlights it as a key frontier for progress toward reliable real-world applications.

==> dkvyckmztzhccsnhttrnhthhdxwytnqw/introduction.tex <==
\section{Introduction}

Large language models (LLMs) now dominate mathematical benchmarks, scoring nearly perfectly on AIME~\citep{openai2024reasoning,guo2025deepseek,openai2025gpt5} and even reaching IMO gold\footnote{\url{https://x.com/alexwei_/status/1946477742855532918}}. Yet these successes remain confined to well‑defined benchmark problems, with little sign of comparable progress on the broader reasoning skills required for real‑world impact~\citep{qian2025modelingagent}.

This gap reflects a fundamental divide in mathematics. On one side are well‑defined abstract problems, such as algebra or analytic geometry, that can be solved through established strategies and symbolic manipulation~\citep{polya1945solve,schoenfeld2014mathematical}. On the other side are scenario‑based problems, ranging from financial analysis to scientific research and engineering design, where the mathematical core is conveyed through concrete narrative detail.  
Existing benchmarks overwhelmingly target the former \citep{cobbe2021gsm8k,lightman2023let,he2024olympiadbench}, leaving the latter largely unexamined. In this work, we term this underexplored domain \textbf{contextual mathematical reasoning}: the ability to formulate and solve the mathematical problem when it is embedded in narrative scenarios with indirect or layered conditions.

To investigate this capability, we introduce \textbf{ContextMATH} (\textbf{Context}ual Reasoning Evaluation for \textbf{Math}), a benchmark designed to probe contextual mathematical reasoning systematically.
Rather than seeking massive collections of real‑world tasks, ContextMATH builds on standard sources—AIME 2024, AIME 2025, and MATH‑500~\citep{lightman2023let}—and instantiates each problem in two controlled narrative variants: 
\textit{Scenario Grounding (SG)} embeds abstract mathematical structures into concrete narratives with real-world entities and interactions. The reasoning core remains unchanged, but the problem is situated in descriptions that naturally introduce contextual detail.  
\textit{Complexity Scaling (CS)} conceals explicit conditions within sub‑problems in the scenario. For example, an absolute position may be given relative to a reference point, or a numerical bound may appear as the result of a short calculation. These sub-problems yield exactly the information originally explicit, while reflecting how constraints are often expressed in real-world settings. This format also reduces reliance on surface pattern matching, since models must first interpret the scenario to recover the original conditions.  
Although demonstrated here for mathematics, the same approach applies to other domains and datasets, enabling systematic evaluation of contextual reasoning beyond math. Figure~\ref{Fig.example} illustrates such mappings; for example, the variables $(a,b,c)$ in the original problem correspond to system components in SG and drone movements in CS.


\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{example.pdf} 
\caption{
Example from ContextMATH, based on AIME 2025 Problem 15. In Scenario Grounding (SG), mathematical components are mapped to a narrative. In Complexity Scaling (CS), explicit conditions are concealed in sub-problems requiring an extra inference step. Consistent color-coding highlights correspondence between mathematical components across the three versions. LLMs remain strong on abstract benchmarks but drop accuracy on SG, with the gap widening further on CS.
}
\label{Fig.example}
\end{figure}

Our results show that both leading open-source and proprietary LLMs experience a substantial decline in contextual mathematical reasoning compared to their strong performance on original benchmarks. On average, open-source models drop 13\% on SG and 34\% on CS, while proprietary models fall 13\% and 20\%, respectively. For example, \texttt{Qwen3-32B} falls from 81.25\% on AIME 2024 problems to 67.92\% on SG and 57.08\% on CS. A similar trend holds for proprietary systems: even \texttt{DeepSeek-R1} drops from 86.67\% to 73.33\% (SG) and 53.33\% (CS) on AIME 2025.

To better understand these limitations, we analyze models’ ability to formulate the mathematical core from narrative scenarios. We find that performance declines as problems become harder, and although larger models perform better, even \texttt{GPT‑5} averages only 81.4\% formulation accuracy. Furthermore, correct formulation proves to be a prerequisite: correctly solved problems show much higher formulation accuracy than average, establishing formulation as the first bottleneck. 
We further observe that as models scale and formulation accuracy improves, correct formulation increasingly becomes sufficient for solution correctness, indicating progress in both problem understanding and reasoning. Yet even \texttt{GPT‑5} reaches only 82.7\% sufficiency, showing that reasoning remains a second major bottleneck for real‑world mathematical problem solving.


We further explore whether the performance drops can be alleviated via training. Our results show that fine-tuning with scenario data effectively improves models' performance on our benchmark, yet a sizable drop on contextual variants still remains, indicating that contextual mathematical reasoning is far from solved. In contrast, directly training a dedicated formulation model proves ineffective, suggesting that formulation ability is difficult to acquire from paired supervision alone.

Our contributions can be summarized as follows:  
\begin{itemize}[leftmargin=1em,labelsep=0.1em,topsep=0.em,itemsep=0.em]
    \item \textbf{New task.} We frame contextual mathematical reasoning, the ability to extract and solve the mathematical core from narrative descriptions, as a critical but underexplored capacity for LLMs.  
    \item \textbf{New benchmark.} We propose \textbf{ContextMATH}, which instantiates problems from AIME and MATH‑500 into Scenario Grounding (SG) and Complexity Scaling (CS) variants to probe mathematical formulation and reasoning under contextual challenges. Evaluations show large accuracy drops on SG and CS relative to abstract benchmarks, revealing a clear and persistent gap between abstract and contextual mathematical reasoning in current LLMs.
    \item \textbf{New insights.} Through quantitative and qualitative analysis, we identify formulation and reasoning as complementary bottlenecks, and provide evidence that training with scenario data improves performance, whereas training a dedicated formulation model remains ineffective. These findings suggest that contextual mathematical reasoning is learnable, but cannot be reduced to isolated skills, highlighting the need for integrated approaches to advance formulation and reasoning.
\end{itemize}



==> dkvyckmztzhccsnhttrnhthhdxwytnqw/main_results.tex <==
\begin{table*}[htbp]
\scriptsize
\centering
% \setlength{\tabcolsep}{4pt}
\sisetup{table-align-text-post=false} % Ensures parentheses are treated correctly
\begin{tabular}{
    l % model
    @{\hspace{2.2pt}}
    S[table-format=2.1] % Ori
    @{\hspace{2.2pt}}
    S[table-format=2.1] % SG
    @{\hspace{1pt}}
    l
    @{\hspace{2.2pt}}
    S[table-format=2.1] % CS
    @{\hspace{1pt}}
    l
    @{\hspace{2.2pt}}
    S[table-format=2.1] % Ori
    @{\hspace{2.2pt}}
    S[table-format=2.1] % SG
    @{\hspace{1pt}}
    l
    @{\hspace{2.2pt}}
    S[table-format=2.1] % CS
    @{\hspace{1pt}}
    l
    @{\hspace{2.2pt}}
    S[table-format=2.1] % Ori
    @{\hspace{2.2pt}}
    S[table-format=2.1] % SG
    @{\hspace{1pt}}
    l
}
\toprule
\multicolumn{1}{l}{\textbf{Model}} & 
\multicolumn{5}{c}{\textbf{AIME2024 (\%)}} & 
\multicolumn{5}{c}{\textbf{AIME2025 (\%)}} & \multicolumn{3}{c}{\textbf{Math-500 (\%)}} \\ 
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-14}
& \multicolumn{1}{c}{\textbf{Ori}} & \multicolumn{2}{c}{\textbf{SG}} & \multicolumn{2}{c}{\textbf{CS}} & \multicolumn{1}{c}{\textbf{Ori}} & \multicolumn{2}{c}{\textbf{SG}} & \multicolumn{2}{c}{\textbf{CS}} & \multicolumn{1}{c}{\textbf{Ori}} & \multicolumn{2}{c}{\textbf{SG}} \\
\midrule
\rowcolor{gray!20}
\multicolumn{14}{c}{\textbf{\textit{$\leq$4B}}} \\
\midrule
Qwen3-0.6B & 7.9 & 6.2 & (\colorbox{PastelRed!21.1}{-21\%}) & 0.4 & (\colorbox{PastelRed!94.7}{-95\%}) & 15.4 & 5.4 & (\colorbox{PastelRed!64.9}{\ \ -65\%}) & 2.5 & (\colorbox{PastelRed!83.8}{\ \ -84\%}) & 62.4 & 42.6 & (\colorbox{PastelRed!31.6}{-32\%}) \\
% Qwen2.5-Math-1.5B-Instruct & 13.3 & 7.9 & (\colorbox{PastelRed!40.6}{-41\%}) & 1.2 & (\colorbox{PastelRed!90.6}{-91\%}) & 10.4 & 4.2 & (\colorbox{PastelRed!60.0}{\ \ -60\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 58.7 & 44.6 & (\colorbox{PastelRed!24.0}{-24\%}) \\
Qwen2.5-Math-1.5B & 11.7 & 2.5 & (\colorbox{PastelRed!78.6}{-79\%}) & 0.4 & (\colorbox{PastelRed!96.4}{-96\%}) & 4.6 & 0.8 & (\colorbox{PastelRed!81.9}{\ \ -82\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 32.5 & 25.8 & (\colorbox{PastelRed!20.7}{-21\%}) \\
\firstarrow R1-Distil-Qwen-1.5B & 28.3 & 20.0 & (\colorbox{PastelRed!29.4}{-29\%}) & 7.1 & (\colorbox{PastelRed!75.0}{-75\%}) & 19.6 & 9.6 & (\colorbox{PastelRed!51.1}{\ \ -51\%}) & 5.8 & (\colorbox{PastelRed!70.2}{\ \ -70\%}) & 74.0 & 57.6 & (\colorbox{PastelRed!22.1}{-22\%}) \\
\secondarrow DeepScaleR-1.5B-Preview & 41.7 & 23.3 & (\colorbox{PastelRed!44.0}{-44\%}) & 7.5 & (\colorbox{PastelRed!82.0}{-82\%}) & 30.4 & 15.4 & (\colorbox{PastelRed!49.3}{\ \ -49\%}) & 7.5 & (\colorbox{PastelRed!75.3}{\ \ -75\%}) & 80.1 & 64.2 & (\colorbox{PastelRed!19.8}{-20\%}) \\
\secondarrow DeepMath-1.5B & 38.3 & 24.6 & (\colorbox{PastelRed!35.9}{-36\%}) & 10.8 & (\colorbox{PastelRed!71.7}{-72\%}) & 28.3 & 13.8 & (\colorbox{PastelRed!51.5}{\ \ -51\%}) & 5.0 & (\colorbox{PastelRed!82.4}{\ \ -82\%}) & 81.9 & 65.4 & (\colorbox{PastelRed!20.2}{-20\%}) \\
\secondarrow Still-3-1.5B-Preview & 38.3 & 18.8 & (\colorbox{PastelRed!51.1}{-51\%}) & 7.9 & (\colorbox{PastelRed!79.3}{-79\%}) & 24.6 & 11.2 & (\colorbox{PastelRed!54.2}{\ \ -54\%}) & 2.5 & (\colorbox{PastelRed!89.8}{\ \ -90\%}) & 75.8 & 59.7 & (\colorbox{PastelRed!21.3}{-21\%}) \\
\firstarrow OpenMath-Nemotron-1.5B & 62.5 & 34.2 & (\colorbox{PastelRed!45.3}{-45\%}) & 14.6 & (\colorbox{PastelRed!76.7}{-77\%}) & 50.4 & 21.2 & (\colorbox{PastelRed!57.9}{\ \ -58\%}) & 11.2 & (\colorbox{PastelRed!77.7}{\ \ -78\%}) & 87.3 & 70.1 & (\colorbox{PastelRed!19.6}{-20\%}) \\
\secondarrow DeepMath-Omn-1.5B & 62.9 & 33.8 & (\colorbox{PastelRed!46.4}{-46\%}) & 13.8 & (\colorbox{PastelRed!78.1}{-78\%}) & 55.8 & 20.8 & (\colorbox{PastelRed!62.7}{\ \ -63\%}) & 12.5 & (\colorbox{PastelRed!77.6}{\ \ -78\%}) & 87.1 & 73.0 & (\colorbox{PastelRed!16.2}{-16\%}) \\
Qwen3-1.7B & 46.2 & 29.6 & (\colorbox{PastelRed!36.0}{-36\%}) & 12.5 & (\colorbox{PastelRed!73.0}{-73\%}) & 34.6 & 24.6 & (\colorbox{PastelRed!28.9}{\ \ -29\%}) & 11.2 & (\colorbox{PastelRed!67.5}{\ \ -67\%}) & 84.1 & 67.4 & (\colorbox{PastelRed!19.9}{-20\%}) \\
Qwen3-4B & 70.4 & 52.5 & (\colorbox{PastelRed!25.4}{-25\%}) & 34.6 & (\colorbox{PastelRed!50.9}{-51\%}) & 64.2 & 39.6 & (\colorbox{PastelRed!38.3}{\ \ -38\%}) & 33.8 & (\colorbox{PastelRed!47.4}{\ \ -47\%}) & 90.9 & 78.8 & (\colorbox{PastelRed!13.3}{-13\%}) \\
\midrule
\rowcolor{gray!20}
\multicolumn{14}{c}{\textbf{\textit{7B/8B}}} \\
\midrule
Qwen2.5-7B & 5.8 & 4.6 & (\colorbox{PastelRed!21.4}{-21\%}) & 1.7 & (\colorbox{PastelRed!71.4}{-71\%}) & 3.3 & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 0.4 & (\colorbox{PastelRed!87.4}{\ \ -87\%}) & 43.9 & 30.4 & (\colorbox{PastelRed!30.7}{-31\%}) \\
\firstarrow Open-Reasoner-Zero-7B & 15.8 & 12.5 & (\colorbox{PastelRed!21.0}{-21\%}) & 6.2 & (\colorbox{PastelRed!60.5}{-61\%}) & 14.6 & 7.1 & (\colorbox{PastelRed!51.4}{\ \ -51\%}) & 2.5 & (\colorbox{PastelRed!82.9}{\ \ -83\%}) & 69.3 & 53.0 & (\colorbox{PastelRed!23.5}{-23\%}) \\
\firstarrow DeepMath-Zero-7B & 18.8 & 7.5 & (\colorbox{PastelRed!60.0}{-60\%}) & 5.8 & (\colorbox{PastelRed!68.9}{-69\%}) & 15.8 & 9.2 & (\colorbox{PastelRed!42.1}{\ \ -42\%}) & 2.1 & (\colorbox{PastelRed!86.9}{\ \ -87\%}) & 74.2 & 59.6 & (\colorbox{PastelRed!19.7}{-20\%}) \\
Qwen2.5-Math-7B & 10.8 & 6.7 & (\colorbox{PastelRed!38.4}{-38\%}) & 1.7 & (\colorbox{PastelRed!84.6}{-85\%}) & 5.0 & 3.3 & (\colorbox{PastelRed!33.4}{\ \ -33\%}) & 0.8 & (\colorbox{PastelRed!83.4}{\ \ -83\%}) & 44.8 & 36.7 & (\colorbox{PastelRed!18.1}{-18\%}) \\
\firstarrow OpenMath-Nemotron-7B & 72.9 & 52.1 & (\colorbox{PastelRed!28.6}{-29\%}) & 30.0 & (\colorbox{PastelRed!58.9}{-59\%}) & 60.0 & 40.4 & (\colorbox{PastelRed!32.6}{\ \ -33\%}) & 29.2 & (\colorbox{PastelRed!51.4}{\ \ -51\%}) & 90.5 & 78.5 & (\colorbox{PastelRed!13.3}{-13\%}) \\
\firstarrow R1-Distil-Qwen-7B & 48.8 & 40.0 & (\colorbox{PastelRed!17.9}{-18\%}) & 23.3 & (\colorbox{PastelRed!52.1}{-52\%}) & 41.7 & 22.5 & (\colorbox{PastelRed!46.0}{\ \ -46\%}) & 15.0 & (\colorbox{PastelRed!64.0}{\ \ -64\%}) & 87.4 & 73.9 & (\colorbox{PastelRed!15.4}{-15\%}) \\
\secondarrow AceMath-RL-Nemotron-7B & 69.2 & 48.8 & (\colorbox{PastelRed!29.5}{-30\%}) & 32.9 & (\colorbox{PastelRed!52.4}{-52\%}) & 54.2 & 26.7 & (\colorbox{PastelRed!50.8}{\ \ -51\%}) & 22.5 & (\colorbox{PastelRed!58.5}{\ \ -58\%}) & 89.9 & 79.0 & (\colorbox{PastelRed!12.2}{-12\%}) \\
\firstarrow Qwen2.5-Math-7B-SRL-Zero & 16.2 & 6.7 & (\colorbox{PastelRed!59.0}{-59\%}) & 0.8 & (\colorbox{PastelRed!94.9}{-95\%}) & 4.6 & 3.3 & (\colorbox{PastelRed!27.3}{\ \ -27\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 49.6 & 33.4 & (\colorbox{PastelRed!32.7}{-33\%}) \\
\firstarrow Qwen2.5-Math-7B-SRL & 20.8 & 14.2 & (\colorbox{PastelRed!32.0}{-32\%}) & 9.2 & (\colorbox{PastelRed!56.0}{-56\%}) & 17.5 & 10.4 & (\colorbox{PastelRed!40.5}{\ \ -40\%}) & 2.9 & (\colorbox{PastelRed!83.3}{\ \ -83\%}) & 70.7 & 58.3 & (\colorbox{PastelRed!17.6}{-18\%}) \\
\firstarrow DeepMath-Zero-Math-7B & 30.4 & 18.8 & (\colorbox{PastelRed!38.4}{-38\%}) & 9.2 & (\colorbox{PastelRed!69.9}{-70\%}) & 22.1 & 15.8 & (\colorbox{PastelRed!28.3}{\ \ -28\%}) & 7.1 & (\colorbox{PastelRed!67.9}{\ \ -68\%}) & 77.4 & 63.8 & (\colorbox{PastelRed!17.6}{-18\%}) \\
\firstarrow Qwen2.5-Math-7B-Oat-Zero & 32.5 & 18.8 & (\colorbox{PastelRed!42.3}{-42\%}) & 2.9 & (\colorbox{PastelRed!91.0}{-91\%}) & 11.2 & 9.2 & (\colorbox{PastelRed!18.5}{\ \ -18\%}) & 0.4 & (\colorbox{PastelRed!96.3}{\ \ -96\%}) & 66.2 & 44.2 & (\colorbox{PastelRed!33.2}{-33\%}) \\
\firstarrow Eurus-2-7B-PRIME-Zero & 20.0 & 13.3 & (\colorbox{PastelRed!33.4}{-33\%}) & 6.7 & (\colorbox{PastelRed!66.6}{-67\%}) & 6.7 & 10.0 & (\colorbox{PastelRed!49.9}{\ \ -50\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 59.9 & 39.7 & (\colorbox{PastelRed!33.8}{-34\%}) \\
\firstarrow Eurus-2-7B-SFT & 6.7 & 3.3 & (\colorbox{PastelRed!50.1}{-50\%}) & 3.3 & (\colorbox{PastelRed!50.1}{-50\%}) & 3.3 & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 50.0 & 38.5 & (\colorbox{PastelRed!22.9}{-23\%}) \\
\secondarrow Eurus-2-7B-PRIME & 20.0 & 13.3 & (\colorbox{PastelRed!33.4}{-33\%}) & 6.7 & (\colorbox{PastelRed!66.6}{-67\%}) & 10.0 & 3.3 & (\colorbox{PastelRed!66.7}{\ \ -67\%}) & 3.3 & (\colorbox{PastelRed!66.7}{\ \ -67\%}) & 68.3 & 57.6 & (\colorbox{PastelRed!15.6}{-16\%}) \\
R1-Distil-Llama-8B & 43.3 & 29.2 & (\colorbox{PastelRed!32.7}{-33\%}) & 10.8 & (\colorbox{PastelRed!75.0}{-75\%}) & 30.4 & 17.5 & (\colorbox{PastelRed!42.5}{\ \ -42\%}) & 11.2 & (\colorbox{PastelRed!63.0}{\ \ -63\%}) & 81.6 & 65.6 & (\colorbox{PastelRed!19.6}{-20\%}) \\
Qwen3-8B & 73.8 & 61.7 & (\colorbox{PastelRed!16.4}{-16\%}) & 42.9 & (\colorbox{PastelRed!41.8}{-42\%}) & 64.6 & 48.3 & (\colorbox{PastelRed!25.2}{\ \ -25\%}) & 35.8 & (\colorbox{PastelRed!44.5}{\ \ -45\%}) & 91.0 & 81.0 & (\colorbox{PastelRed!11.0}{-11\%}) \\
\firstarrow DeepSeek-R1-0528-Qwen3-8B & 75.0 & 55.0 & (\colorbox{PastelRed!26.7}{-27\%}) & 39.6 & (\colorbox{PastelRed!47.2}{-47\%}) & 65.8 & 48.3 & (\colorbox{PastelRed!26.6}{\ \ -27\%}) & 32.9 & (\colorbox{PastelRed!50.0}{\ \ -50\%}) & 90.7 & 77.2 & (\colorbox{PastelRed!14.9}{-15\%}) \\
\firstarrow AReaL-boba-2-8B & 74.2 & 58.3 & (\colorbox{PastelRed!21.4}{-21\%}) & 41.7 & (\colorbox{PastelRed!43.8}{-44\%}) & 67.9 & 47.9 & (\colorbox{PastelRed!29.4}{\ \ -29\%}) & 37.1 & (\colorbox{PastelRed!45.4}{\ \ -45\%}) & 91.8 & 82.0 & (\colorbox{PastelRed!10.7}{-11\%}) \\
Qwen2.5-Math-7B-Instruct & 11.2 & 6.2 & (\colorbox{PastelRed!44.4}{-44\%}) & 2.5 & (\colorbox{PastelRed!77.8}{-78\%}) & 9.2 & 5.0 & (\colorbox{PastelRed!45.5}{\ \ -45\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 72.0 & 54.0 & (\colorbox{PastelRed!25.0}{-25\%}) \\
\midrule
\rowcolor{gray!20}
\multicolumn{14}{c}{\textbf{\textit{14B}}} \\
\midrule
Qwen2.5-14B & 6.2 & 3.8 & (\colorbox{PastelRed!40.0}{-40\%}) & 1.7 & (\colorbox{PastelRed!73.3}{-73\%}) & 3.3 & 1.7 & (\colorbox{PastelRed!49.8}{\ \ -50\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 48.5 & 34.9 & (\colorbox{PastelRed!28.1}{-28\%}) \\
\firstarrow R1-Distil-Qwen-14B & 67.5 & 47.1 & (\colorbox{PastelRed!30.3}{-30\%}) & 35.4 & (\colorbox{PastelRed!47.5}{-48\%}) & 50.8 & 26.2 & (\colorbox{PastelRed!48.4}{\ \ -48\%}) & 25.8 & (\colorbox{PastelRed!49.2}{\ \ -49\%}) & 89.5 & 76.9 & (\colorbox{PastelRed!14.0}{-14\%}) \\
\firstarrow OpenMath-Nemotron-14B & 73.8 & 51.7 & (\colorbox{PastelRed!29.9}{-30\%}) & 42.1 & (\colorbox{PastelRed!42.9}{-43\%}) & 63.8 & 42.5 & (\colorbox{PastelRed!33.3}{\ \ -33\%}) & 29.2 & (\colorbox{PastelRed!54.2}{\ \ -54\%}) & 90.8 & 80.8 & (\colorbox{PastelRed!11.0}{-11\%}) \\
Qwen3-14B & 80.0 & 64.6 & (\colorbox{PastelRed!19.3}{-19\%}) & 50.8 & (\colorbox{PastelRed!36.5}{-36\%}) & 72.9 & 49.2 & (\colorbox{PastelRed!32.6}{\ \ -33\%}) & 42.1 & (\colorbox{PastelRed!42.3}{\ \ -42\%}) & 92.6 & 81.9 & (\colorbox{PastelRed!11.5}{-12\%}) \\
\firstarrow AReaL-boba-2-14B & 82.9 & 65.8 & (\colorbox{PastelRed!20.6}{-21\%}) & 53.8 & (\colorbox{PastelRed!35.2}{-35\%}) & 73.3 & 52.1 & (\colorbox{PastelRed!29.0}{\ \ -29\%}) & 39.2 & (\colorbox{PastelRed!46.6}{\ \ -47\%}) & 91.9 & 82.9 & (\colorbox{PastelRed!9.9}{-10\%}) \\
Phi-4-reasoning-plus & 80.4 & 60.4 & (\colorbox{PastelRed!24.9}{-25\%}) & 52.9 & (\colorbox{PastelRed!34.2}{-34\%}) & 71.7 & 55.4 & (\colorbox{PastelRed!22.7}{\ \ -22\%}) & 39.6 & (\colorbox{PastelRed!44.8}{\ \ -45\%}) & 92.6 & 83.1 & (\colorbox{PastelRed!10.3}{-10\%}) \\
\midrule
\rowcolor{gray!20}
\multicolumn{14}{c}{\textbf{\textit{$\ge$32B }}} \\
\midrule
Qwen2.5-32B & 11.2 & 6.7 & (\colorbox{PastelRed!40.7}{-41\%}) & 3.3 & (\colorbox{PastelRed!70.4}{-70\%}) & 3.8 & 2.9 & (\colorbox{PastelRed!22.1}{\ \ -22\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 45.2 & 37.8 & (\colorbox{PastelRed!16.4}{-16\%}) \\
\firstarrow OpenMath-Nemotron-32B & 57.1 & 42.5 & (\colorbox{PastelRed!25.5}{-26\%}) & 27.9 & (\colorbox{PastelRed!51.1}{-51\%}) & 52.1 & 34.6 & (\colorbox{PastelRed!33.6}{\ \ -34\%}) & 27.5 & (\colorbox{PastelRed!47.2}{\ \ -47\%}) & 75.8 & 61.8 & (\colorbox{PastelRed!18.5}{-18\%}) \\
\firstarrow R1-Distil-Qwen-32B & 69.6 & 52.5 & (\colorbox{PastelRed!24.5}{-25\%}) & 39.2 & (\colorbox{PastelRed!43.7}{-44\%}) & 56.2 & 39.6 & (\colorbox{PastelRed!29.6}{\ \ -30\%}) & 30.0 & (\colorbox{PastelRed!46.7}{\ \ -47\%}) & 89.4 & 78.9 & (\colorbox{PastelRed!11.8}{-12\%}) \\
\firstarrow Open-Reasoner-Zero-32B & 43.8 & 30.4 & (\colorbox{PastelRed!30.5}{-30\%}) & 25.4 & (\colorbox{PastelRed!41.9}{-42\%}) & 32.9 & 25.4 & (\colorbox{PastelRed!22.6}{\ \ -23\%}) & 15.0 & (\colorbox{PastelRed!54.4}{\ \ -54\%}) & 84.3 & 75.1 & (\colorbox{PastelRed!10.9}{-11\%}) \\
Qwen3-32B & \second{81.2} & \best{67.9} & (\colorbox{PastelRed!16.4}{-16\%}) & \second{57.1} & (\colorbox{PastelRed!29.7}{-30\%}) & \second{70.0} & \second{54.4} & (\colorbox{PastelRed!22.3}{\ \ -22\%}) & \best{45.0} & (\colorbox{PastelRed!35.7}{\ \ -36\%}) &  92.1 & \second{82.7} & (\colorbox{PastelRed!10.3}{-10\%}) \\
\firstarrow AReaL-boba-2-32B & 81.7 & 65.4 & (\colorbox{PastelRed!19.9}{-20\%}) & 58.3 & (\colorbox{PastelRed!28.6}{-29\%}) & 77.1 & 55.0 & (\colorbox{PastelRed!28.6}{\ \ -29\%}) & 43.8 & (\colorbox{PastelRed!43.2}{\ \ -43\%}) & 92.3 & 82.9 & (\colorbox{PastelRed!10.2}{-10\%}) \\
QwQ-32B & 80.4 & 58.3 & (\colorbox{PastelRed!27.5}{-27\%}) & 53.3 & (\colorbox{PastelRed!33.7}{-34\%}) & 66.2 & 53.3 & (\colorbox{PastelRed!19.5}{\ \ -20\%}) & 39.2 & (\colorbox{PastelRed!40.9}{\ \ -41\%}) & 92.5 & 82.9 & (\colorbox{PastelRed!10.4}{-10\%}) \\
Qwen2.5-32B-Instruct & 15.4 & 14.2 & (\colorbox{PastelRed!8.1}{\ \ -8\%}) & 5.4 & (\colorbox{PastelRed!64.9}{-65\%}) & 15.8 & 9.2 & (\colorbox{PastelRed!42.1}{\ \ -42\%}) & 1.7 & (\colorbox{PastelRed!89.5}{\ \ -89\%}) & 70.3 & 54.5 & (\colorbox{PastelRed!22.5}{-23\%}) \\
\firstarrow s1.1-32B & 58.8 & 47.9 & (\colorbox{PastelRed!18.4}{-18\%}) & 38.3 & (\colorbox{PastelRed!34.8}{-35\%}) & 46.7 & 36.2 & (\colorbox{PastelRed!22.3}{\ \ -22\%}) & 32.1 & (\colorbox{PastelRed!31.3}{\ \ -31\%}) & 88.8 & 77.9 & (\colorbox{PastelRed!12.3}{-12\%}) \\
DeepSeek-R1-Distill-Llama-70B & 65.4 & 48.8 & (\colorbox{PastelRed!25.5}{-25\%}) & 38.8 & (\colorbox{PastelRed!40.8}{-41\%}) & 50.0 & 38.8 & (\colorbox{PastelRed!22.5}{\ \ -22\%}) & 29.2 & (\colorbox{PastelRed!41.7}{\ \ -42\%}) & 89.8 & 77.3 & (\colorbox{PastelRed!14.0}{-14\%}) \\
Qwen2.5-Math-72B-Instruct & 19.2 & 13.8 & (\colorbox{PastelRed!28.3}{-28\%}) & 6.7 & (\colorbox{PastelRed!65.2}{-65\%}) & 14.6 & 7.5 & (\colorbox{PastelRed!48.6}{\ \ -49\%}) & 3.3 & (\colorbox{PastelRed!77.2}{\ \ -77\%}) & 74.7 & 60.5 & (\colorbox{PastelRed!19.0}{-19\%}) \\
\bottomrule
\end{tabular}
\caption{Full results of open‑source models on ContextMATH. Models are grouped by parameter scale. 
Parentheses indicate the relative change from Ori, with larger drops highlighted by deeper red. 
Arrows ($\firstarrow$) denote variants obtained from the model listed directly above.}
\label{tab:model_performance}
\end{table*}



==> dkvyckmztzhccsnhttrnhthhdxwytnqw/main_results_short.tex <==
\begin{table*}[t]
\scriptsize
\centering
% \setlength{\tabcolsep}{4pt}
% \sisetup{table-align-text-post=false} % Ensures parentheses are treated correctly
\begin{tabular}{
    l % model
    @{\hspace{1.5pt}}
    S[table-format=2.1] % Q0
    @{\hspace{1.5pt}}
    S[table-format=2.1] % Q1
    @{\hspace{0.8pt}}
    l
    @{\hspace{1.5pt}}
    S[table-format=2.1] % Q2
    @{\hspace{0.8pt}}
    l
    @{\hspace{1.5pt}}
    S[table-format=2.1] % Q0
    @{\hspace{1.5pt}}
    S[table-format=2.1] % Q1
    @{\hspace{0.8pt}}
    l
    @{\hspace{1.5pt}}
    S[table-format=2.1] % Q2
    @{\hspace{0.8pt}}
    l
    @{\hspace{1.5pt}}
    S[table-format=2.1] % Q0
    @{\hspace{1.5pt}}
    S[table-format=2.1] % Q1
    @{\hspace{0.8pt}}
    l
}
\toprule
\multicolumn{1}{l}{\textbf{Model}} & 
\multicolumn{5}{c}{\textbf{AIME 2024 (\%)}} & 
\multicolumn{5}{c}{\textbf{AIME 2025 (\%)}} & \multicolumn{3}{c}{\textbf{Math-500 (\%)}} \\ 
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-14}
& \multicolumn{1}{c}{\textbf{Ori}} & \multicolumn{2}{c}{\textbf{SG}} & \multicolumn{2}{c}{\textbf{CS}} & \multicolumn{1}{c}{\textbf{Ori}} & \multicolumn{2}{c}{\textbf{SG}} & \multicolumn{2}{c}{\textbf{CS}} & \multicolumn{1}{c}{\textbf{Ori}} & \multicolumn{2}{c}{\textbf{SG}} \\
\midrule
\rowcolor{gray!20}
\multicolumn{14}{c}{\textbf{\textit{$\leq$4B}}} \\
\midrule
Qwen3-0.6B & 7.9 & 6.2 & (\colorbox{PastelRed!21.1}{-21\%}) & 0.4 & (\colorbox{PastelRed!94.7}{-95\%}) & 15.4 & 5.4 & (\colorbox{PastelRed!64.9}{-65\%}) & 2.5 & (\colorbox{PastelRed!83.8}{\ \ -84\%}) & 62.4 & 42.6 & (\colorbox{PastelRed!31.6}{-32\%}) \\
Qwen2.5-Math-1.5B & 11.5 & 2.5 & (\colorbox{PastelRed!78.6}{-79\%}) & 0.4 & (\colorbox{PastelRed!96.4}{-96\%}) & 4.6 & 0.8 & (\colorbox{PastelRed!81.9}{-82\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 32.5 & 25.8 & (\colorbox{PastelRed!20.7}{-21\%}) \\
\firstarrow R1-Distil-Qwen-1.5B & 28.3 & 20.0 & (\colorbox{PastelRed!29.4}{-29\%}) & 7.1 & (\colorbox{PastelRed!75.0}{-75\%}) & 19.6 & 9.6 & (\colorbox{PastelRed!51.1}{-51\%}) & 5.8 & (\colorbox{PastelRed!70.2}{\ \ -70\%}) & 74.0 & 57.6 & (\colorbox{PastelRed!22.1}{-22\%}) \\
\secondarrow DeepScaleR-1.5B-Preview & 41.5 & 23.3 & (\colorbox{PastelRed!44.0}{-44\%}) & 7.5 & (\colorbox{PastelRed!82.0}{-82\%}) & 30.4 & 15.4 & (\colorbox{PastelRed!49.3}{-49\%}) & 7.5 & (\colorbox{PastelRed!75.3}{\ \ -75\%}) & 80.1 & 64.2 & (\colorbox{PastelRed!19.8}{-20\%}) \\
\firstarrow OpenMath-Nemotron-1.5B & 62.5 & \second{34.2} & (\colorbox{PastelRed!45.3}{-45\%}) & \second{14.6} & (\colorbox{PastelRed!76.7}{-77\%}) & 50.4 & 21.2 & (\colorbox{PastelRed!57.9}{-58\%}) & 11.2 & (\colorbox{PastelRed!77.7}{\ \ -78\%}) & \second{87.3} & 70.1 & (\colorbox{PastelRed!19.6}{-20\%}) \\
\secondarrow DeepMath-Omn-1.5B & \second{62.9} & 33.8 & (\colorbox{PastelRed!46.4}{-46\%}) & 13.8 & (\colorbox{PastelRed!78.1}{-78\%}) & \second{55.8} & 20.8 & (\colorbox{PastelRed!62.7}{-63\%}) & \second{12.5} & (\colorbox{PastelRed!77.6}{\ \ -78\%}) & 87.1 & \second{73.0} & (\colorbox{PastelRed!16.2}{-16\%}) \\
Qwen3-1.5B & 46.2 & 29.6 & (\colorbox{PastelRed!36.0}{-36\%}) & 12.5 & (\colorbox{PastelRed!73.0}{-73\%}) & 34.6 & \second{24.6} & (\colorbox{PastelRed!28.9}{-29\%}) & 11.2 & (\colorbox{PastelRed!67.5}{\ \ -67\%}) & 84.1 & 67.4 & (\colorbox{PastelRed!19.9}{-20\%}) \\
Qwen3-4B & \best{70.4} & \best{52.5} & (\colorbox{PastelRed!25.4}{-25\%}) & \best{34.6} & (\colorbox{PastelRed!50.9}{-51\%}) & \best{64.2} & \best{39.6} & (\colorbox{PastelRed!38.3}{-38\%}) & \best{33.8} & (\colorbox{PastelRed!47.4}{\ \ -47\%}) & \best{90.9} & \best{78.8} & (\colorbox{PastelRed!13.3}{-13\%}) \\
\midrule
\rowcolor{gray!20}
\multicolumn{14}{c}{\textbf{\textit{7B/8B}}} \\
\midrule
Qwen2.5-Math-7B & 10.8 & 6.7 & (\colorbox{PastelRed!38.4}{-38\%}) & 1.5 & (\colorbox{PastelRed!84.6}{-85\%}) & 5.0 & 3.3 & (\colorbox{PastelRed!33.4}{-33\%}) & 0.8 & (\colorbox{PastelRed!83.4}{\ \ -83\%}) & 44.8 & 36.7 & (\colorbox{PastelRed!18.1}{-18\%}) \\
\firstarrow OpenMath-Nemotron-7B & 72.9 & 52.1 & (\colorbox{PastelRed!28.6}{-29\%}) & 30.0 & (\colorbox{PastelRed!58.9}{-59\%}) & 60.0 & 40.4 & (\colorbox{PastelRed!32.6}{-33\%}) & 29.2 & (\colorbox{PastelRed!51.4}{\ \ -51\%}) & 90.5 & 78.5 & (\colorbox{PastelRed!13.3}{-13\%}) \\
\firstarrow R1-Distil-Qwen-7B & 48.8 & 40.0 & (\colorbox{PastelRed!17.9}{-18\%}) & 23.3 & (\colorbox{PastelRed!52.1}{-52\%}) & 41.5 & 22.5 & (\colorbox{PastelRed!46.0}{-46\%}) & 15.0 & (\colorbox{PastelRed!64.0}{\ \ -64\%}) & 87.4 & 73.9 & (\colorbox{PastelRed!15.4}{-15\%}) \\
\secondarrow AceMath-RL-Nemotron-7B & 69.2 & 48.8 & (\colorbox{PastelRed!29.5}{-30\%}) & 32.9 & (\colorbox{PastelRed!52.4}{-52\%}) & 54.2 & 26.7 & (\colorbox{PastelRed!50.8}{-51\%}) & 22.5 & (\colorbox{PastelRed!58.5}{\ \ -58\%}) & 89.9 & 79.0 & (\colorbox{PastelRed!12.2}{-12\%}) \\
% R1-Distil-Llama-8B & 43.3 & 29.2 & (\colorbox{PastelRed!32.7}{-33\%}) & 10.8 & (\colorbox{PastelRed!75.0}{-75\%}) & 30.4 & 17.5 & (\colorbox{PastelRed!42.5}{-42\%}) & 11.2 & (\colorbox{PastelRed!63.0}{\ \ -63\%}) & 81.6 & 65.6 & (\colorbox{PastelRed!19.6}{-20\%}) \\
Qwen3-8B & 73.8 & \best{61.5} & (\colorbox{PastelRed!16.4}{-16\%}) & \best{42.9} & (\colorbox{PastelRed!41.5}{-42\%}) & 64.6 & \best{48.3} & (\colorbox{PastelRed!25.2}{-25\%}) & \second{35.8} & (\colorbox{PastelRed!44.5}{\ \ -45\%}) & \second{91.0} & \second{81.0} & (\colorbox{PastelRed!11.0}{-11\%}) \\
\firstarrow R1-0528-Qwen3-8B & \best{75.0} & 55.0 & (\colorbox{PastelRed!26.7}{-27\%}) & 39.6 & (\colorbox{PastelRed!47.2}{-47\%}) & \second{65.8} & \best{48.3} & (\colorbox{PastelRed!26.6}{-27\%}) & 32.9 & (\colorbox{PastelRed!50.0}{\ \ -50\%}) & 90.7 & 77.2 & (\colorbox{PastelRed!14.9}{-15\%}) \\
\firstarrow AReaL-boba-2-8B & \second{74.2} & \second{58.3} & (\colorbox{PastelRed!21.4}{-21\%}) & \second{41.5} & (\colorbox{PastelRed!43.8}{-44\%}) & \best{67.9} & \second{47.9} & (\colorbox{PastelRed!29.4}{-29\%}) & \best{37.1} & (\colorbox{PastelRed!45.4}{\ \ -45\%}) & \best{91.5} & \best{82.0} & (\colorbox{PastelRed!10.7}{-11\%}) \\
\midrule
\rowcolor{gray!20}
\multicolumn{14}{c}{\textbf{\textit{14B}}} \\
\midrule
Qwen2.5-14B & 6.2 & 3.8 & (\colorbox{PastelRed!40.0}{-40\%}) & 1.5 & (\colorbox{PastelRed!73.3}{-73\%}) & 3.3 & 1.5 & (\colorbox{PastelRed!49.8}{-50\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 48.5 & 34.9 & (\colorbox{PastelRed!28.1}{-28\%}) \\
\firstarrow R1-Distil-Qwen-14B & 67.5 & 47.1 & (\colorbox{PastelRed!30.3}{-30\%}) & 35.4 & (\colorbox{PastelRed!47.5}{-48\%}) & 50.8 & 26.2 & (\colorbox{PastelRed!48.4}{-48\%}) & 25.8 & (\colorbox{PastelRed!49.2}{\ \ -49\%}) & 89.5 & 76.9 & (\colorbox{PastelRed!14.0}{-14\%}) \\
\firstarrow OpenMath-Nemotron-14B & 73.8 & 51.5 & (\colorbox{PastelRed!29.9}{-30\%}) & 42.1 & (\colorbox{PastelRed!42.9}{-43\%}) & 63.8 & 42.5 & (\colorbox{PastelRed!33.3}{-33\%}) & 29.2 & (\colorbox{PastelRed!54.2}{\ \ -54\%}) & 90.8 & 80.8 & (\colorbox{PastelRed!11.0}{-11\%}) \\
Qwen3-14B & 80.0 & \second{64.6} & (\colorbox{PastelRed!19.3}{-19\%}) & 50.8 & (\colorbox{PastelRed!36.5}{-36\%}) & \second{72.9} & 49.2 & (\colorbox{PastelRed!32.6}{-33\%}) & \best{42.1} & (\colorbox{PastelRed!42.3}{\ \ -42\%}) & \best{92.6} & 81.9 & (\colorbox{PastelRed!11.5}{-12\%}) \\
\firstarrow AReaL-boba-2-14B & \best{82.9} & \best{65.8} & (\colorbox{PastelRed!20.6}{-21\%}) & \best{53.8} & (\colorbox{PastelRed!35.2}{-35\%}) & \best{73.3} & \second{52.1} & (\colorbox{PastelRed!29.0}{-29\%}) & 39.2 & (\colorbox{PastelRed!46.6}{\ \ -47\%}) & \second{91.9} & \second{82.9} & (\colorbox{PastelRed!9.9}{-10\%}) \\
Phi-4-reasoning-plus & \second{80.4} & 60.4 & (\colorbox{PastelRed!24.9}{-25\%}) & \second{52.9} & (\colorbox{PastelRed!34.2}{-34\%}) & 71.5 & \best{55.4} & (\colorbox{PastelRed!22.7}{-22\%}) & \second{39.6} & (\colorbox{PastelRed!44.8}{\ \ -45\%}) & \best{92.6} & \best{83.1} & (\colorbox{PastelRed!10.3}{-10\%}) \\
\midrule
\rowcolor{gray!20}
\multicolumn{14}{c}{\textbf{\textit{$\ge$32B }}} \\
\midrule
Qwen2.5-32B & 11.2 & 6.7 & (\colorbox{PastelRed!40.7}{-41\%}) & 3.3 & (\colorbox{PastelRed!70.4}{-70\%}) & 3.8 & 2.9 & (\colorbox{PastelRed!22.1}{-22\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) & 45.2 & 37.8 & (\colorbox{PastelRed!16.4}{-16\%}) \\
\firstarrow OpenMath-Nemotron-32B & 57.1 & 42.5 & (\colorbox{PastelRed!25.5}{-26\%}) & 27.9 & (\colorbox{PastelRed!51.1}{-51\%}) & 52.1 & 34.6 & (\colorbox{PastelRed!33.6}{-34\%}) & 27.5 & (\colorbox{PastelRed!47.2}{\ \ -47\%}) & 75.8 & 61.8 & (\colorbox{PastelRed!18.5}{-18\%}) \\
\firstarrow R1-Distil-Qwen-32B & 69.6 & 52.5 & (\colorbox{PastelRed!24.5}{-25\%}) & 39.2 & (\colorbox{PastelRed!43.7}{-44\%}) & 56.2 & 39.6 & (\colorbox{PastelRed!29.6}{-30\%}) & 30.0 & (\colorbox{PastelRed!46.7}{\ \ -47\%}) & 89.4 & 78.9 & (\colorbox{PastelRed!11.5}{-12\%}) \\
Qwen3-32B & \second{81.2} & \best{67.9} & (\colorbox{PastelRed!16.4}{-16\%}) & \second{57.1} & (\colorbox{PastelRed!29.7}{-30\%}) & \second{70.0} & \second{54.4} & (\colorbox{PastelRed!22.3}{-22\%}) & \best{45.0} & (\colorbox{PastelRed!35.7}{\ \ -36\%}) &  92.1 & \second{82.7} & (\colorbox{PastelRed!10.3}{-10\%}) \\
\firstarrow AReaL-boba-2-32B & \best{81.5} & \second{65.4} & (\colorbox{PastelRed!19.9}{-20\%}) & \best{58.3} & (\colorbox{PastelRed!28.6}{-29\%}) & \best{77.1} & \best{55.0} & (\colorbox{PastelRed!28.6}{-29\%}) & \second{43.8} & (\colorbox{PastelRed!43.2}{\ \ -43\%}) & \second{92.3} & \best{82.9} & (\colorbox{PastelRed!10.2}{-10\%}) \\
QwQ-32B & 80.4 & 58.3 & (\colorbox{PastelRed!27.5}{-27\%}) & 53.3 & (\colorbox{PastelRed!33.7}{-34\%}) & 66.2 & 53.3 & (\colorbox{PastelRed!19.5}{-20\%}) & 39.2 & (\colorbox{PastelRed!40.9}{\ \ -41\%}) & \best{92.5} & \best{82.9} & (\colorbox{PastelRed!10.4}{-10\%}) \\
R1-Distill-Llama-70B & 65.4 & 48.8 & (\colorbox{PastelRed!25.5}{-25\%}) & 38.8 & (\colorbox{PastelRed!40.8}{-41\%}) & 50.0 & 38.8 & (\colorbox{PastelRed!22.5}{-22\%}) & 29.2 & (\colorbox{PastelRed!41.5}{\ \ -42\%}) & 89.8 & 77.3 & (\colorbox{PastelRed!14.0}{-14\%}) \\
\bottomrule
\end{tabular}
\caption{
Accuracy of open-source models on ContextMATH. Models are grouped by parameter scale, and best and second-best results within each group are shown in \textbf{bold} and \underline{underlined}, respectively. Parentheses indicate the relative performance change from Ori, with larger drops highlighted by a deeper shade of red. Arrows ($\firstarrow$) denote variants obtained from the model listed directly above. 
Full results are provided in Appendix~\ref{app:opensource_results}.
}
\label{tab:model_performance_short}
\end{table*}


==> dkvyckmztzhccsnhttrnhthhdxwytnqw/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> dkvyckmztzhccsnhttrnhthhdxwytnqw/pro_model_results.tex <==
\begin{table*}[t]
\scriptsize
\centering
% \setlength{\tabcolsep}{6pt}
\sisetup{table-align-text-post=false} % Ensures parentheses are treated correctly
\sisetup{table-number-alignment=center} % Ensures parentheses are treated correctly
\begin{tabular}{
    l % model
    @{\hspace{13pt}}
    S[table-format=2.1] % Q0
    @{\hspace{13pt}}
    S[table-format=2.1] % Q1
    @{\hspace{1pt}}
    l
    @{\hspace{13pt}}
    S[table-format=2.1] % Q1 pass@3
    @{\hspace{1pt}}
    l
    @{\hspace{13pt}}
    S[table-format=2.1] % Q2
    @{\hspace{1pt}}
    l
    @{\hspace{13pt}}
    S[table-format=2.1] % Q0
    @{\hspace{13pt}}
    S[table-format=2.1] % Q1
    @{\hspace{1pt}}
    l
    @{\hspace{13pt}}
    S[table-format=2.1] % Q2
    @{\hspace{1pt}}
    l
}
\toprule
\multicolumn{1}{l}{\textbf{Model}} & 
\multicolumn{7}{c}{\textbf{AIME 2024 (\%)}} & 
\multicolumn{5}{c}{\textbf{AIME 2025 (\%)}} \\ 
\cmidrule(lr){2-8} \cmidrule(lr){9-13}
& \multicolumn{1}{c}{\hspace{-2em}\textbf{Ori}} & \multicolumn{2}{c}{\hspace{-2em}\textbf{SG}} & \multicolumn{2}{c}{\hspace{-2em}\textbf{SG Avg@3}} & \multicolumn{2}{c}{\hspace{-2em}\textbf{CS}} & \multicolumn{1}{c}{\hspace{-2em}\textbf{Ori}} & \multicolumn{2}{c}{\hspace{-2em}\textbf{SG}} & \multicolumn{2}{c}{\hspace{-2em}\textbf{CS}} \\
\midrule
Copilot & 30.0 & 30.0 & (\colorbox{PastelRed!0}{\ \ -0\%}) & 28.9 & (\colorbox{PastelRed!3.7}{\ \ -4\%}) & 23.3 & (\colorbox{PastelRed!22.2}{-22\%}) & 33.3 & 20.0 & (\colorbox{PastelRed!40.0}{-40\%}) & 16.7 & (\colorbox{PastelRed!50.0}{\ \ -50\%}) \\
gpt-4o-mini & 6.7 & 3.3 & (\colorbox{PastelRed!50.1}{-50\%}) & 6.7 & (\colorbox{PastelRed!0}{\ \ -0\%}) & 3.3 & (\colorbox{PastelRed!50.1}{-50\%}) & 10.0 & 6.7 & (\colorbox{PastelRed!33.3}{-33\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) \\
o1-mini & 60.0 & 53.3 & (\colorbox{PastelRed!11.1}{-11\%}) & 53.3 & (\colorbox{PastelRed!11}{-11\%}) & 40.0 & (\colorbox{PastelRed!33.3}{-33\%}) & 40.0 & 33.3 & (\colorbox{PastelRed!16.7}{-17\%}) & 23.3 & (\colorbox{PastelRed!41.7}{\ \ -42\%}) \\
gpt-4o & 16.7 & 13.3 & (\colorbox{PastelRed!20.0}{-20\%}) & 11.1 & (\colorbox{PastelRed!33.4}{-33\%}) &  3.3 & (\colorbox{PastelRed!80.0}{-80\%}) & 10.0 & 6.7 & (\colorbox{PastelRed!33.3}{-33\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) \\
gpt-4.1-mini & 46.7 & 26.7 & (\colorbox{PastelRed!42.9}{-43\%}) & 34.4 & (\colorbox{PastelRed!26.2}{-26\%}) & 30.0 & (\colorbox{PastelRed!35.7}{-36\%}) & 53.3 & 30.0 & (\colorbox{PastelRed!43.7}{-44\%}) & 16.7 & (\colorbox{PastelRed!68.7}{\ \ -69\%}) \\
gpt-4.1-nano & 26.7 & 23.3 & (\colorbox{PastelRed!12.5}{-13\%}) & 18.9 & (\colorbox{PastelRed!29.2}{-29\%}) & 6.7 & (\colorbox{PastelRed!75.0}{-75\%}) & 33.3 & 20.0 & (\colorbox{PastelRed!40.0}{-40\%}) & 13.3 & (\colorbox{PastelRed!60.0}{\ \ -60\%}) \\
R1 & \best{93.3} & 70.0 & (\colorbox{PastelRed!25.0}{-25\%}) & 70.0 & (\colorbox{PastelRed!25.0}{-25\%}) & 66.7 & (\colorbox{PastelRed!28.6}{-29\%}) & \second{86.7} & \second{73.3} & (\colorbox{PastelRed!15.4}{-15\%}) & 53.3 & (\colorbox{PastelRed!38.5}{\ \ -38\%}) \\
Doubao-1.5 & \second{90.0} & 70.0 & (\colorbox{PastelRed!22.2}{-22\%}) & 66.7 & (\colorbox{PastelRed!25.9}{-26\%}) & 56.7 & (\colorbox{PastelRed!37.0}{-37\%}) & 76.7 & 53.3 & (\colorbox{PastelRed!30.4}{-30\%}) & 43.3 & (\colorbox{PastelRed!43.5}{\ \ -43\%}) \\
Qwen-max & 23.3 & 16.7 & (\colorbox{PastelRed!28.5}{-29\%}) & 14.4 & (\colorbox{PastelRed!38.1}{-38\%}) & 6.7 & (\colorbox{PastelRed!71.4}{-71\%}) & 13.3 & 10.0 & (\colorbox{PastelRed!25.0}{-25\%}) & 0.0 & (\colorbox{PastelRed!100.0}{-100\%}) \\
QwQ-plus & 86.7 & 56.7 & (\colorbox{PastelRed!34.6}{-35\%}) & 60.0 & (\colorbox{PastelRed!30.8}{-31\%}) &  46.7 & (\colorbox{PastelRed!46.2}{-46\%}) & 73.3 & 53.3 & (\colorbox{PastelRed!27.3}{-27\%}) & 43.3 & (\colorbox{PastelRed!40.9}{\ \ -41\%}) \\
Grok3 & 43.3 & 23.3 & (\colorbox{PastelRed!46.2}{-46\%}) & 22.2 & (\colorbox{PastelRed!48.7}{-49\%}) & 23.3 & (\colorbox{PastelRed!46.2}{-46\%}) & 26.7 & 13.3 & (\colorbox{PastelRed!50.0}{-50\%}) & 20.0 & (\colorbox{PastelRed!25.0}{\ \ -25\%}) \\
Gemini 2.5 Flash & 70.0 & 63.3 & (\colorbox{PastelRed!9.5}{-10\%}) & 61.1 & (\colorbox{PastelRed!12.7}{-13\%}) & 53.3 & (\colorbox{PastelRed!23.8}{-24\%}) & 70.0 & 43.3 & (\colorbox{PastelRed!38.1}{-38\%}) & 30.0 & (\colorbox{PastelRed!57.1}{\ \ -57\%}) \\
Gemini 2.5 Pro & 83.3 & \second{73.3} & (\colorbox{PastelRed!12.0}{-12\%}) & 68.9 & (\colorbox{PastelRed!17.3}{-17\%}) & \second{76.7} & (\colorbox{PastelRed!8.0}{\ \ -8\%}) & 83.3 & 56.7 & (\colorbox{PastelRed!32.0}{-32\%}) & 50.0 & (\colorbox{PastelRed!40.0}{\ \ -40\%}) \\
o3 & 83.3 & 70.0 & (\colorbox{PastelRed!16.0}{-16\%}) & \second{73.3} & (\colorbox{PastelRed!12.0}{-12\%}) & 66.7 & (\colorbox{PastelRed!20.0}{-20\%}) & 76.7 & 70.0 & (\colorbox{PastelRed!8.7}{\ \ -9\%}) & \second{60.0} & (\colorbox{PastelRed!21.7}{\ \ -22\%}) \\
gpt-5 & \second{90.0} & \best{83.3} & (\colorbox{PastelRed!7.4}{\ \ -7\%}) & \best{82.2} & (\colorbox{PastelRed!8.6}{\ \ -9\%}) & \best{80.0} & (\colorbox{PastelRed!11.1}{-11\%}) & \best{90.0} & \best{80.0} & (\colorbox{PastelRed!11.1}{-11\%}) & \best{66.7} & (\colorbox{PastelRed!25.9}{\ \ -26\%}) \\
\bottomrule
\end{tabular}
\caption{
Accuracy of proprietary models on ContextMATH. Best and second-best results per column are in \textbf{bold} and \underline{underlined}, respectively. Parentheses indicate the relative performance change from Ori, with larger drops highlighted in a deeper shade of red.
To verify that our findings are consistent and not an artifact of specific scenarios, we additionally generated and annotated two AIME2024-SG sets, reporting the average accuracy across all three in the \texttt{SG Avg@3} column.
}
\label{tab:proprietary_model_performance}
\end{table*}




==> dkvyckmztzhccsnhttrnhthhdxwytnqw/quantitative.tex <==
\begin{table}[H]
\centering
\scriptsize
\setlength{\tabcolsep}{1.4pt}
\begin{tabular}{l cc cc c cc cc c cc cc c}
\toprule
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{Formulation Accuracy (\%)}} & \multicolumn{5}{c}{\textbf{Formulation Necessity (\%)}} & \multicolumn{5}{c}{\textbf{Formulation Sufficiency (\%)}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
& \multicolumn{2}{c}{\textbf{AIME24}} & \multicolumn{2}{c}{\textbf{AIME25}} & \textbf{MATH} & \multicolumn{2}{c}{\textbf{AIME24}} & \multicolumn{2}{c}{\textbf{AIME25}} & \textbf{MATH} & \multicolumn{2}{c}{\textbf{AIME24}} & \multicolumn{2}{c}{\textbf{AIME25}} & \textbf{MATH} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11}
& \textbf{SG} & \textbf{CS} & \textbf{SG} & \textbf{CS} & \textbf{SG} & \textbf{SG} & \textbf{CS} & \textbf{SG} & \textbf{CS} & \textbf{SG} & \textbf{SG} & \textbf{CS} & \textbf{SG} & \textbf{CS} & \textbf{SG} \\
\midrule
R1-Distil-Qwen-1.5B & \colorbox{lightyellow!53.6}{57.5} & \colorbox{lightyellow!28.6}{40.0} & \colorbox{lightyellow!41.7}{49.2} & \colorbox{lightyellow!16.7}{31.7} & \colorbox{lightyellow!60.4}{62.3} & \colorbox{MintGreen!28.6}{61.4} & \colorbox{MintGreen!15.0}{\ \ 43.8} & \colorbox{MintGreen!15.0}{41.7} & \colorbox{MintGreen!62.5}{75.0} & \colorbox{MintGreen!51.5}{70.6} & \colorbox{BabyBlue!10}{17.5} & \colorbox{BabyBlue!5}{10.1} & \colorbox{BabyBlue!5}{9.1} & \colorbox{BabyBlue!5}{15.9} & \colorbox{BabyBlue!62.6}{65.0} \\
R1-Distil-Qwen-7B & \colorbox{lightyellow!57.1}{60.0} & \colorbox{lightyellow!51.2}{55.8} & \colorbox{lightyellow!47.6}{53.3} & \colorbox{lightyellow!29.8}{40.8} & \colorbox{lightyellow!79.5}{75.7} & \colorbox{MintGreen!44.5}{67.8} & \colorbox{MintGreen!40.6}{\ \ 66.2} & \colorbox{MintGreen!33.1}{63.2} & \colorbox{MintGreen!20.8}{58.3} & \colorbox{MintGreen!82.2}{82.9} & \colorbox{BabyBlue!15.9}{46.3} & \colorbox{BabyBlue!10}{31.1} & \colorbox{BabyBlue!10}{26.7} & \colorbox{BabyBlue!10}{22.2} & \colorbox{BabyBlue!100.0}{81.1} \\
R1-Distil-Qwen-14B & \colorbox{lightyellow!77.4}{74.2} & \colorbox{lightyellow!61.9}{63.3} & \colorbox{lightyellow!47.6}{53.3} & \colorbox{lightyellow!42.9}{50.0} & \colorbox{lightyellow!93.8}{85.7} & \colorbox{MintGreen!77.0}{80.8} & \colorbox{MintGreen!54.2}{\ \ 71.7} & \colorbox{MintGreen!70.8}{78.3} & \colorbox{MintGreen!78.3}{81.3} & \colorbox{MintGreen!100.0}{90.1} & \colorbox{BabyBlue!34.1}{53.7} & \colorbox{BabyBlue!5.6}{42.2} & \colorbox{BabyBlue!10}{31.7} & \colorbox{BabyBlue!5.8}{42.3} & \colorbox{BabyBlue!100.0}{80.8} \\
R1-Distil-Qwen-32B & \colorbox{lightyellow!82.1}{77.5} & \colorbox{lightyellow!65.5}{65.8} & \colorbox{lightyellow!56.0}{59.2} & \colorbox{lightyellow!57.1}{60.0} & \colorbox{lightyellow!96.2}{87.3} & \colorbox{MintGreen!75.2}{80.1} & \colorbox{MintGreen!67.5}{\ \ 77.0} & \colorbox{MintGreen!49.6}{69.8} & \colorbox{MintGreen!70.0}{78.0} & \colorbox{MintGreen!100.0}{91.8} & \colorbox{BabyBlue!29.2}{51.7} & \colorbox{BabyBlue!14.9}{45.9} & \colorbox{BabyBlue!15.3}{46.1} & \colorbox{BabyBlue!0.0}{39.4} & \colorbox{BabyBlue!100.0}{83.5} \\
Qwen3-0.6B & \colorbox{lightyellow!38.1}{46.7} & \colorbox{lightyellow!13.1}{29.2} & \colorbox{lightyellow!36.9}{45.8} & \colorbox{lightyellow!21.4}{35.0} & \colorbox{lightyellow!53.5}{57.4} & \colorbox{MintGreen!25.0}{52.8} & \colorbox{MintGreen!100.0}{100.0} & \colorbox{MintGreen!10.0}{33.3} & \colorbox{MintGreen!8.0}{25.0} & \colorbox{MintGreen!47.9}{69.2} & \colorbox{BabyBlue!5}{\ \ 8.4} & \colorbox{BabyBlue!5}{\ \ 3.6} & \colorbox{BabyBlue!5}{\ \ 1.5} & \colorbox{BabyBlue!5}{\ \ 1.9} & \colorbox{BabyBlue!30.4}{52.2} \\
Qwen3-1.7B & \colorbox{lightyellow!66.7}{66.7} & \colorbox{lightyellow!39.3}{47.5} & \colorbox{lightyellow!57.1}{60.0} & \colorbox{lightyellow!47.6}{53.3} & \colorbox{lightyellow!89.3}{82.5} & \colorbox{MintGreen!59.3}{73.7} & \colorbox{MintGreen!86.3}{\ \ 84.5} & \colorbox{MintGreen!45.9}{68.4} & \colorbox{MintGreen!83.3}{83.3} & \colorbox{MintGreen!100.0}{90.1} & \colorbox{BabyBlue!10}{32.4} & \colorbox{BabyBlue!10}{24.8} & \colorbox{BabyBlue!10}{27.6} & \colorbox{BabyBlue!10}{14.1} & \colorbox{BabyBlue!84.4}{73.8} \\
Qwen3-4B & \colorbox{lightyellow!77.4}{74.2} & \colorbox{lightyellow!50.0}{55.0} & \colorbox{lightyellow!45.2}{51.7} & \colorbox{lightyellow!32.1}{42.5} & \colorbox{lightyellow!92.6}{84.8} & \colorbox{MintGreen!100.0}{91.1} & \colorbox{MintGreen!74.8}{\ \ 79.9} & \colorbox{MintGreen!34.4}{63.7} & \colorbox{MintGreen!52.6}{71.0} & \colorbox{MintGreen!100.0}{90.3} & \colorbox{BabyBlue!63.7}{65.5} & \colorbox{BabyBlue!22.1}{48.8} & \colorbox{BabyBlue!26.7}{50.7} & \colorbox{BabyBlue!44.5}{57.8} & \colorbox{BabyBlue!100.0}{83.6} \\
Qwen3-8B & \colorbox{lightyellow!88.1}{81.7} & \colorbox{lightyellow!77.4}{74.2} & \colorbox{lightyellow!66.7}{66.7} & \colorbox{lightyellow!57.1}{60.0} & \colorbox{lightyellow!94.7}{86.3} & \colorbox{MintGreen!99.5}{89.8} & \colorbox{MintGreen!83.9}{\ \ 83.6} & \colorbox{MintGreen!68.1}{77.3} & \colorbox{MintGreen!67.9}{77.2} & \colorbox{MintGreen!100.0}{91.3} & \colorbox{BabyBlue!65.1}{66.0} & \colorbox{BabyBlue!23.3}{49.3} & \colorbox{BabyBlue!35.6}{54.2} & \colorbox{BabyBlue!19.3}{47.7} & \colorbox{BabyBlue!100.0}{86.3} \\
Qwen3-14B & \colorbox{lightyellow!82.1}{77.5} & \colorbox{lightyellow!69.0}{68.3} & \colorbox{lightyellow!66.7}{66.7} & \colorbox{lightyellow!60.7}{62.5} & \colorbox{lightyellow!95.9}{87.1} & \colorbox{MintGreen!80.3}{82.1} & \colorbox{MintGreen!62.0}{\ \ 74.8} & \colorbox{MintGreen!77.5}{81.0} & \colorbox{MintGreen!100.0}{95.8} & \colorbox{MintGreen!100.0}{90.4} & \colorbox{BabyBlue!61.6}{64.6} & \colorbox{BabyBlue!43.5}{57.4} & \colorbox{BabyBlue!56.1}{62.4} & \colorbox{BabyBlue!55.0}{62.0} & \colorbox{BabyBlue!100.0}{85.2} \\
Qwen3-32B & \colorbox{lightyellow!91.7}{84.2} & \colorbox{lightyellow!71.4}{70.0} & \colorbox{lightyellow!75.0}{72.5} & \colorbox{lightyellow!56.0}{59.2} & \colorbox{lightyellow!99.0}{89.3} & \colorbox{MintGreen!76.1}{80.5} & \colorbox{MintGreen!60.1}{\ \ 74.0} & \colorbox{MintGreen!90.5}{86.2} & \colorbox{MintGreen!66.6}{76.6} & \colorbox{MintGreen!100.0}{92.0} & \colorbox{BabyBlue!66.1}{66.4} & \colorbox{BabyBlue!48.9}{59.6} & \colorbox{BabyBlue!43.8}{57.5} & \colorbox{BabyBlue!39.3}{55.7} & \colorbox{BabyBlue!100.0}{85.0} \\
% gpt-4o & \colorbox{lightyellow!71.4}{70.0} & \colorbox{lightyellow!33.3}{43.3} & \colorbox{lightyellow!28.6}{40.0} & \colorbox{lightyellow!9.5}{26.7} & & \colorbox{MintGreen!62.5}{75.0} & \colorbox{MintGreen!0.0}{0.0} & \colorbox{MintGreen!0.0}{50.0} & \colorbox{MintGreen!0.0}{0.0} & \\
% gpt-4.1-mini & \colorbox{lightyellow!95.2}{86.7} & \colorbox{lightyellow!85.7}{80.0} & \colorbox{lightyellow!71.4}{70.0} & \colorbox{lightyellow!33.3}{43.3} & & \colorbox{MintGreen!93.8}{87.5} & \colorbox{MintGreen!69.4}{77.8} & \colorbox{MintGreen!100.0}{100.0} & \colorbox{MintGreen!75.0}{80.0} & & \colorbox{BabyBlue!0.0}{26.9} & \colorbox{BabyBlue!0.0}{29.2} & \colorbox{BabyBlue!7.1}{42.9} & \colorbox{BabyBlue!0.0}{30.8} & \\
% o1-mini & \colorbox{lightyellow!100.0}{90.0} & \colorbox{lightyellow!61.9}{63.3} & \colorbox{lightyellow!76.2}{73.3} & \colorbox{lightyellow!47.6}{53.3} & & \colorbox{MintGreen!100.0}{93.8} & \colorbox{MintGreen!20.8}{58.3} & \colorbox{MintGreen!0.0}{50.0} & \colorbox{MintGreen!17.9}{57.1} &  \\
gpt-5 & \colorbox{lightyellow!100.0}{93.3} & \colorbox{lightyellow!81.0}{76.7} & \colorbox{lightyellow!85.7}{80.0} & \colorbox{lightyellow!66.7}{66.7} & \colorbox{lightyellow!100.0}{90.5} & \colorbox{MintGreen!100.0}{96.0} & \colorbox{MintGreen!72.9}{\ \ 79.2} & \colorbox{MintGreen!83.3}{83.3} & \colorbox{MintGreen!62.5}{75.0} & \colorbox{MintGreen!100.0}{94.5}  & \colorbox{BabyBlue!100.0}{85.7} & \colorbox{BabyBlue!100.0}{82.6} & \colorbox{BabyBlue!100.0}{83.3} & \colorbox{BabyBlue!87.5}{75.0} & \colorbox{BabyBlue!100.0}{86.9} \\
\bottomrule
\end{tabular}
\caption{
Problem formulation performance comparison across different models. Formulation Accuracy denotes the proportion of cases in which a model correctly translates a scenario into its mathematical formulation. Formulation Necessity quantifies the extent to which correct formulations are required for correct reasoning. Formulation Sufficiency evaluates whether correct formulations reliably lead to correct reasoning. Darker cell colors correspond to higher values.
}
\label{appx:formulation_results}
\end{table}


==> dkvyckmztzhccsnhttrnhthhdxwytnqw/quantitative_merged.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{
    l
    c@{\hspace{3pt}}cc@{\hspace{9pt}}c
    @{\hspace{8pt}}
    c@{\hspace{3pt}}cc@{\hspace{9pt}}c
    @{\hspace{8pt}}
    c@{\hspace{3pt}}cc@{\hspace{9pt}}c
}
\toprule
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{Formulation Accuracy (\%)}} & \multicolumn{4}{c}{\textbf{Formulation Necessity (\%)}} & \multicolumn{4}{c}{\textbf{Formulation Sufficiency (\%)}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
& \textbf{MATH} & \multicolumn{1}{c}{\textbf{AIME24}} & \multicolumn{1}{c}{\textbf{AIME25}} & \textbf{Avg.} & \textbf{MATH} & \multicolumn{1}{c}{\textbf{AIME24}} & \multicolumn{1}{c}{\textbf{AIME25}} & \textbf{Avg.} & \textbf{MATH} & \multicolumn{1}{c}{\textbf{AIME24}} & \multicolumn{1}{c}{\textbf{AIME25}} & \textbf{Avg.} \\
\midrule
R1-Distill-Qwen-1.5B & \colorbox{lightyellow!53.8}{62.3} & \colorbox{lightyellow!31.2}{48.8} & \colorbox{lightyellow!17.4}{40.4} & \colorbox{lightyellow!30.2}{48.1} & \colorbox{MintGreen!61.2}{70.6} & \colorbox{MintGreen!25.2}{52.6} & \colorbox{MintGreen!36.7}{58.3} & \colorbox{MintGreen!37.0}{58.5} & \colorbox{BabyBlue!70.1}{65.0} & \colorbox{BabyBlue!0.0}{13.8} & \colorbox{BabyBlue!0.0}{12.5} & \colorbox{BabyBlue!0.0}{23.5} \\
R1-Distill-Qwen-7B & \colorbox{lightyellow!76.1}{75.7} & \colorbox{lightyellow!46.5}{57.9} & \colorbox{lightyellow!28.5}{47.1} & \colorbox{lightyellow!45.2}{57.1} & \colorbox{MintGreen!85.7}{82.9} & \colorbox{MintGreen!54.0}{67.0} & \colorbox{MintGreen!41.6}{60.8} & \colorbox{MintGreen!55.4}{67.7} & \colorbox{BabyBlue!100.0}{81.1} & \colorbox{BabyBlue!17.4}{38.7} & \colorbox{BabyBlue!0.0}{24.5} & \colorbox{BabyBlue!23.0}{41.5} \\
R1-Distill-Qwen-14B & \colorbox{lightyellow!92.8}{85.7} & \colorbox{lightyellow!64.6}{68.8} & \colorbox{lightyellow!36.1}{51.7} & \colorbox{lightyellow!58.8}{65.3} & \colorbox{MintGreen!100.0}{90.1} & \colorbox{MintGreen!72.5}{76.2} & \colorbox{MintGreen!79.7}{79.8} & \colorbox{MintGreen!80.9}{80.4} & \colorbox{BabyBlue!100.0}{80.8} & \colorbox{BabyBlue!35.9}{47.9} & \colorbox{BabyBlue!14.1}{37.0} & \colorbox{BabyBlue!40.3}{50.1} \\
R1-Distill-Qwen-32B & \colorbox{lightyellow!95.5}{87.3} & \colorbox{lightyellow!69.4}{71.7} & \colorbox{lightyellow!49.3}{59.6} & \colorbox{lightyellow!66.6}{70.0} & \colorbox{MintGreen!100.0}{91.8} & \colorbox{MintGreen!77.1}{78.5} & \colorbox{MintGreen!67.8}{73.9} & \colorbox{MintGreen!78.7}{79.3} & \colorbox{BabyBlue!100.0}{83.5} & \colorbox{BabyBlue!37.6}{48.8} & \colorbox{BabyBlue!25.5}{42.7} & \colorbox{BabyBlue!46.6}{53.3} \\
Qwen3-0.6B & \colorbox{lightyellow!45.7}{57.4} & \colorbox{lightyellow!13.2}{37.9} & \colorbox{lightyellow!17.4}{40.4} & \colorbox{lightyellow!21.4}{42.8} & \colorbox{MintGreen!58.3}{69.2} & \colorbox{MintGreen!72.8}{76.4} & \colorbox{MintGreen!0.0}{29.2} & \colorbox{MintGreen!32.1}{56.1} & \colorbox{BabyBlue!44.3}{52.2} & \colorbox{BabyBlue!0.0}{6.0} & \colorbox{BabyBlue!0.0}{1.7} & \colorbox{BabyBlue!0.0}{13.5} \\
Qwen3-1.7B & \colorbox{lightyellow!87.6}{82.5} & \colorbox{lightyellow!45.1}{57.1} & \colorbox{lightyellow!44.4}{56.7} & \colorbox{lightyellow!53.3}{62.0} & \colorbox{MintGreen!100.0}{90.1} & \colorbox{MintGreen!78.3}{79.1} & \colorbox{MintGreen!71.7}{75.8} & \colorbox{MintGreen!80.0}{80.0} & \colorbox{BabyBlue!87.5}{73.8} & \colorbox{BabyBlue!0.0}{28.6} & \colorbox{BabyBlue!0.0}{20.8} & \colorbox{BabyBlue!9.0}{34.5} \\
Qwen3-4B & \colorbox{lightyellow!91.4}{84.8} & \colorbox{lightyellow!57.6}{64.6} & \colorbox{lightyellow!28.5}{47.1} & \colorbox{lightyellow!52.7}{61.6} & \colorbox{MintGreen!100.0}{90.3} & \colorbox{MintGreen!91.0}{85.5} & \colorbox{MintGreen!54.8}{67.4} & \colorbox{MintGreen!78.4}{79.2} & \colorbox{BabyBlue!100.0}{83.6} & \colorbox{BabyBlue!54.3}{57.1} & \colorbox{BabyBlue!48.5}{54.2} & \colorbox{BabyBlue!62.5}{61.3} \\
Qwen3-8B & \colorbox{lightyellow!93.8}{86.3} & \colorbox{lightyellow!79.9}{77.9} & \colorbox{lightyellow!55.6}{63.3} & \colorbox{lightyellow!72.9}{73.8} & \colorbox{MintGreen!100.0}{91.3} & \colorbox{MintGreen!93.4}{86.7} & \colorbox{MintGreen!74.4}{77.2} & \colorbox{MintGreen!87.6}{83.8} & \colorbox{BabyBlue!100.0}{86.3} & \colorbox{BabyBlue!55.4}{57.7} & \colorbox{BabyBlue!42.0}{51.0} & \colorbox{BabyBlue!61.4}{60.7} \\
Qwen3-14B & \colorbox{lightyellow!95.2}{87.1} & \colorbox{lightyellow!71.5}{72.9} & \colorbox{lightyellow!57.6}{64.6} & \colorbox{lightyellow!70.7}{72.4} & \colorbox{MintGreen!100.0}{90.4} & \colorbox{MintGreen!76.9}{78.5} & \colorbox{MintGreen!96.8}{88.4} & \colorbox{MintGreen!89.6}{84.8} & \colorbox{BabyBlue!100.0}{85.2} & \colorbox{BabyBlue!62.0}{61.0} & \colorbox{BabyBlue!64.4}{62.2} & \colorbox{BabyBlue!72.7}{66.3} \\
Qwen3-32B & \colorbox{lightyellow!98.9}{89.3} & \colorbox{lightyellow!78.5}{77.1} & \colorbox{lightyellow!59.7}{65.8} & \colorbox{lightyellow!75.0}{75.0} & \colorbox{MintGreen!100.0}{92.0} & \colorbox{MintGreen!74.5}{77.2} & \colorbox{MintGreen!82.8}{81.4} & \colorbox{MintGreen!83.7}{81.9} & \colorbox{BabyBlue!100.0}{85.0} & \colorbox{BabyBlue!66.0}{63.0} & \colorbox{BabyBlue!53.2}{56.6} & \colorbox{BabyBlue!69.7}{64.9} \\
gpt5 & \colorbox{lightyellow!100.0}{90.5} & \colorbox{lightyellow!91.7}{85.0} & \colorbox{lightyellow!72.2}{73.3} & \colorbox{lightyellow!85.7}{81.4} & \colorbox{MintGreen!100.0}{94.5} & \colorbox{MintGreen!95.2}{87.6} & \colorbox{MintGreen!78.3}{79.2} & \colorbox{MintGreen!91.2}{85.6} & \colorbox{BabyBlue!100.0}{86.9} & \colorbox{BabyBlue!100.0}{84.2} & \colorbox{BabyBlue!98.3}{79.2} & \colorbox{BabyBlue!100.0}{82.7} \\
\bottomrule
\end{tabular}
\caption{
Problem formulation performance across different models. Formulation Accuracy denotes how often a model correctly translates a scenario into its formulation. Formulation Necessity quantifies the extent to which correct formulations are required for correct reasoning, while Formulation Sufficiency evaluates whether correct formulations reliably lead to correct reasoning. The AIME24 and AIME25 columns show the average of their SG and CS sets, while the ‘Avg.’ column is the mean over all sets. Darker cell colors indicate higher values.
}
\label{tab:formulation_results}
\end{table}



==> dkvyckmztzhccsnhttrnhthhdxwytnqw/related_work.tex <==
\section{Related Work}
% \subsection{Mathematical Reasoning Benchmarks}
% % 常见纯文本数学 benchmark 介绍
% % GSM8K, Math, AIME, xxx
% % 然而，都是 focus 在数学上的，而无法体现模型在现实生活中对于数学能力的应用
% The research community has developed a variety of benchmarks to measure the mathematical reasoning abilities of LLMs.
% While benchmarks such as GSM8K, MATH and AIME cover diverse topics, their problem statements are generally clear, well-structured, and formal, allowing models to focus solely on the solution process.

% \subsection{Enhancing LLMs' Real-world Performance}
% % 现实能力（数学）
% % 视觉+数学能力：mathvista, chartqa, infvqa
% % 常识+数学：ScienceQA
% % 数据+数学：FinQA, TAT-QA, HiTab
% % 然而这些对数学能力的要求并不要，只需要进行一些简单的运算即可
% % 现有的 benchmark 依旧无法衡量 sota 模型在现实场景下应用复杂数学逻辑的能力
% % 比如即使 sota 模型在数学 benchmark 中表现很好，当面对现实场景中的复杂数学运算问题时，依然会大幅性能下降

% % 现实能力（其他）
% % agent: gaia, agentbench, mind2web
% % OS: OSWorld, OSBench
% % Code: SWE-Bench

\paragraph{Benchmarks on Abstract Mathematical Problems.}
Much of the progress in evaluating LLMs’ mathematical ability has been driven by benchmarks centered on abstract, well-specified problems. GSM8K~\citep{cobbe2021trainingverifierssolvemath} covers grade school arithmetic word problems, while MATH~\citep{hendrycks2021measuringmathematicalproblemsolving} spans high-school curricula, and AIME, AMC23, and OlympiadBench~\citep{he2024olympiadbench} emphasize challenging competition-style questions. 
There are also benchmarks that target formal theorem proving, such as PutnamBench~\citep{tsoukalas2024putnambench}, LeanDojo~\citep{yang2023leandojo}, and MiniF2F~\citep{zheng2021minif2f}. While some existing problems contain simple narratives such as “Jack had 8 pens and Mary had 5 pens…,”~\citep{patel2021nlp} these contexts are shallow and limited in scope. As such, current benchmarks primarily capture performance on clearly formulated abstract problems, leaving open the question of how well models can reason about mathematics when it is embedded in richer contexts.

\paragraph{From Abstract Problems to Scenarios.}
Across domains, a growing line of work has begun to examine model reasoning in realistic settings. For example, WebArena~\citep{zhou2024webarenarealisticwebenvironment} evaluates agents in interactive web environments, while SWE-bench~\citep{jimenez2024swebench} and BaxBench~\citep{vero2025baxbench} focus on real-world software engineering tasks.  
Our work falls within this broader scope, but focuses specifically on mathematical reasoning in scenarios.

% Closer to mathematics, FinQA~\citep{chen2021finqa} and TAT-QA~\citep{zhu-etal-2021-tat} place quantitative reasoning within financial reports, and HiTab~\citep{cheng-etal-2022-hitab} studies reasoning over hierarchical tables. However, these datasets emphasize more on document comprehension, and are constructed from real-world sources, which makes them less scalable. We instead adopt a synthetic approach, building on existing mathematical benchmarks to systematically construct datasets that are specifically designed for studying mathematical reasoning in scenarios.

% \subsection{Contextual and Real-World Reasoning Benchmarks}
% A series of benchmarks have been developed to embed mathematical reasoning within narrative, document-based, or multimodal contexts. FinQA \citep{chen2021finqa}, TAT-QA \citep{zhu-etal-2021-tat}, and HiTab \citep{cheng-etal-2022-hitab} situate quantitative reasoning within financial documents and hierarchical tables. Extending beyond text, ChartQA \citep{masry-etal-2022-chartqa} and MathVista \citep{lu2024mathvista} require models to reason over visual and multimodal inputs. Collectively, these benchmarks emphasize the necessity of integrating comprehension with computation. Yet, they mainly wrap mathematical problems in auxiliary contexts, yielding tasks that resemble textbook-style exercises rather than challenges grounded in real-world environments.

% In contrast, a growing line of work explicitly targets real-world problem solving. GAIA \citep{zavras2025gaiaglobalmultimodalmultiscale} evaluates general-purpose reasoning that integrates information retrieval, tool use, and multimodal inputs. WebArena \citep{zhou2024webarenarealisticwebenvironment} introduces interactive web environments to test agents on realistic multi-step workflows. SWE-bench \citep{jimenez2024swebench} turns to software engineering, requiring models to resolve actual GitHub issues through code modifications validated by unit tests. These benchmarks expose the limitations of current LLMs, which continue to struggle on tasks that demand robust reasoning in realistic settings. This motivates us to investigate models’ mathematical capabilities in genuinely applied environments, moving beyond textbook questions toward scenarios that reflect the demands of practice.



% \subsection{Contextual and Real-World Reasoning Benchmarks}
% A line of benchmarks has been developed that frame mathematical reasoning within narrative, document-based, or multimodal contexts. FinQA \citep{chen2021finqa}, TAT-QA \citep{zhu-etal-2021-tat}, and HiTab \citep{cheng-etal-2022-hitab} situate quantitative reasoning within financial documents and hierarchical tables. Extending beyond text, ChartQA \citep{masry-etal-2022-chartqa} and MathVista \citep{lu2024mathvista} require models to reason over visual and multimodal inputs. Collectively, these benchmarks underscore the need to integrate comprehension with computation. Yet the mathematical demands they impose remain relatively shallow, since most tasks reduce to arithmetic, comparison, or aggregation rather than deeper abstraction or formal modeling.

% Beyond contextualization, some benchmarks directly target real-world problem solving. GAIA \citep{zavras2025gaiaglobalmultimodalmultiscale} targets general-purpose problem solving that integrates information retrieval, tool use, and multimodal reasoning. WebArena \citep{zhou2024webarenarealisticwebenvironment} creates interactive web environments to evaluate agents on realistic multi-step workflows. SWE-bench \citep{jimenez2024swebench} turns to software engineering, requiring models to resolve real GitHub issues through code changes validated by unit tests. 
% Taken together, these benchmarks highlight the persistent limitations of LLMs in addressing real-world tasks. Inspired by this observation, we seek to investigate models’ capacity to confront mathematics in truly applied settings.

% Together, these efforts demonstrate the expanding capacity of LLMs to engage with complex tasks and highlight directions for future progress. 
% Still, when it comes to mathematics, there remains a notable shortfall: few benchmarks extend mathematical competence into contextual or real-world settings. This limitation motivates the development of \textsc{XXX}.


% Recent work has begun to address reasoning in richer contexts. For instance, MathHay \citep{wang2024mathhay} introduces long-context mathematical reasoning tasks where LLMs must locate relevant information across large documents before performing calculations. MathChat \citep{zhenwen2024mathchat} frames multi-turn dialogue math problems that emphasize instruction following and interaction. System-2 Mathematical Reasoning via Enriched Instruction Tuning (EIT) \citep{cai2024eit} improves performance by augmenting datasets with detailed reasoning plans and intermediate steps.  

% These advances suggest progress toward more realistic mathematical reasoning, but they share consistent limitations: they do not systematically vary narrative complexity or test model’s ability to formulate mathematical structure when conditions are only implicitly specified in a narrative. Thus the capability of LLMs to perform true mathematical modeling from narrative remains underexplored.


% \subsection{Methods for Improving Contextual Reasoning}
% Orthogonal to dataset development, recent research has explored methods to improve reasoning capabilities in large language models. Supervised fine-tuning and distillation approaches leverage high-quality reasoning traces, such as chain-of-thought demonstrations, to enhance controllability and stability during inference \citep{wei2023chainofthoughtpromptingelicitsreasoning}. By exposing models to explicit intermediate steps, these methods encourage more faithful reasoning trajectories.  

% Reinforcement learning has also been applied to strengthen multi-step reasoning. Approaches such as GRPO \citep{shao2024deepseekmathpushinglimitsmathematical} and DAPO \citep{yu2025dapoopensourcellmreinforcement} have substantially improved mathematical performance, enabling models to achieve strong results even on challenging benchmarks such as AIME. Yet, while these advances highlight the potential of RL in boosting mathematical competence, existing evaluations remain largely confined to standardized problem sets. The ability of such models to perform complex mathematical reasoning in realistic narrative environments is still underexplored, underscoring the need for dedicated benchmarks.  





==> dkvyckmztzhccsnhttrnhthhdxwytnqw/training.tex <==
\section{Improving Contextual Mathematical Reasoning}

Our analysis in Section~\ref{analysis} reveals two bottlenecks: (i) formulating the mathematical core from a scenario, and (ii) carrying out the subsequent reasoning. In this section, we explore training strategies addressing these challenges, through both end‑to‑end fine‑tuning and dedicated formulation models.

\subsection{End-to-End Training}
\label{sec:sft}
\paragraph{Data.}
(i) \textbf{Original Data}:  
We use DeepMath-103K~\citep{deepmath}, a large-scale dataset of challenging mathematical problems spanning Algebra, Calculus, and Geometry. Each problem is paired with three solutions generated by \texttt{DeepSeek R1}; we randomly sample one per problem as the reference solution.  
(ii) \textbf{Synthetic Scenarios}:  
We generate contextual scenarios for DeepMath problems following the procedure in Section~\ref{benchmark}. To enable scalable data generation without manual verification, we use \texttt{Qwen3-32B} to solve the generated scenarios and retain only those whose final answers match the original problems, ensuring a high likelihood of equivalence. This yields $50k$ validated contextual problems with model-provided reference solutions. For fairness, we also restrict the original dataset to the corresponding $50k$ subset when training.

% \vspace{-2mm}
\paragraph{Experimental Setup.}  
We fine‑tune the \texttt{Qwen3‑Base} series under three training regimes for controlled comparison:  
(1) original data only (+$\text{SFT}_{\text{Ori}}$, $50k$),  
(2) synthetic scenario data only (+$\text{SFT}_{\text{Syn}}$, $50k$), and  
(3) a balanced mixture of both (+$\text{SFT}_{\text{Mix}}$, $100k$).  
All settings are trained with the same number of steps for a fair comparison.  
In addition to our own benchmark, we further evaluate models on AMC23 and Math‑Perturb~\citep{huang2025math} to assess whether the improvements generalize beyond our benchmark. AMC23 measures abstract mathematical reasoning independent of contextualization. Math‑Perturb tests generalization under data shifts, with two variants derived from level‑5 MATH problems~\citep{hendrycks2021measuring}: \emph{Simple}, which alters only non‑critical surface parameters (e.g., numbers), and \emph{Hard}, which modifies the underlying mathematical core.  
Implementation details are provided in Appendix~\ref{implementation details}.


\input{SFT_results}

% \vspace{-2mm}
\paragraph{Results}  
Table~\ref{tab:sft_main_results} shows that SFT markedly boosts contextual reasoning, e.g., \texttt{Qwen3‑14B‑Base} solves only $11.0\%$ of AIME 2024‑SG problems, but rises to $52.5\%$ with $\text{SFT}_{\text{Mix}}$.
Comparing regimes, scenario supervision ($\text{SFT}_{\text{Syn.}}$) is more effective than original problems ($\text{SFT}_{\text{Ori.}}$) on contextual problems, showing that models must see narratives explicitly to acquire this skill. The mixture regime ($\text{SFT}_{\text{Mix}}$) provides the best overall balance—achieving the strongest averages across all sizes—suggesting complementarity between abstract and scenario data.  
Beyond our benchmark, models also improve on AMC23 and Math‑Perturb, indicating that targeted scenario training does not degrade abstract reasoning and even enhances robustness to distribution shifts. Larger models benefit more from scenario supervision, but even with $\text{SFT}_{\text{Mix}}$ they solve under 40\% of AIME 2024/25-CS problems, highlighting both clear progress and substantial remaining headroom.


\subsection{Training a Dedicated Formulation Model}

With formulation identified as a bottleneck, a natural question is whether a model trained solely for formulation, combined with an existing solver, can improve contextual reasoning. This experiment offers a preliminary test of that idea.

% \vspace{-2mm}
\paragraph{Data.}  
We use scenario–original pairs from Section~\ref{sec:sft}, where each training instance maps a contextual scenario to its equivalent abstract problem.  

% \vspace{-2mm}
\paragraph{Experimental Setup.}  
We fine‑tune \texttt{Qwen3‑8B} and \texttt{Qwen3‑14B} as \emph{formulation models}, and also employ them as \emph{reasoning models}. We compare three settings:  
(i) \textbf{w/o formulation}: the reasoning model solves the scenario directly;  
(ii) \textbf{w/ formulation, training‑free}: the formulation model is used without fine‑tuning, and its output is solved by the reasoning model;  
(iii) \textbf{w/ formulation, trained}: the formulation model is fine‑tuned on scenario–original pairs before handing outputs to the reasoning model.  
At evaluation, we sample one formulation per scenario and report the average accuracy of 16 reasoning outputs.
% Training follows exactly the same setup as Appendix~\ref{implementation details}.
Implementation details are provided in Appendix~\ref{implementation details}.

\input{two_stage_results}
% \vspace{-2mm}
\paragraph{Results.}
As shown in Table~\ref{tab:two_stage_results}, the best performance comes from solving scenarios directly (\textbf{w/o formulation}). Adding an untuned formulation stage leads to a slight drop, indicating that the pipeline introduces extra errors that propagate to reasoning. With a tuned formulation model, performance collapses further. Since training is stable and shows no signs of overfitting, we conclude that formulation is difficult to learn effectively from scenario–original pairs alone, and we leave the exploration of other approaches to future work.

==> dkvyckmztzhccsnhttrnhthhdxwytnqw/two_stage_results.tex <==
\begin{wraptable}{h}{0.42\textwidth}
\vspace{-4mm}
\centering
\scriptsize
\setlength{\tabcolsep}{5.8pt}
\begin{tabular}{l cccccc}
\toprule
\multirow{3}{*}{\textbf{\makecell{Reasoning \\ Model}}} & \multicolumn{5}{c}{\textbf{Formulation Model (Qwen3-8/14B)}} \\
\cmidrule(lr){2-6}
& \multirow{2}{*}{\textbf{w/o}} & \multicolumn{2}{c}{\textbf{Untuned}} & \multicolumn{2}{c}{\textbf{Tuned}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & \textbf{8B} & \textbf{14B} & \textbf{8B} & \textbf{14B} \\ 
\midrule
Qwen3-8B & 53.9 & 48.9 & 53.4 & 20.8 & 22.3 \\
Qwen3-14B & 57.7 & 51.8 & 56.2 & 21.8 & 24.6 \\

\bottomrule
\end{tabular}
\caption{
Average accuracy on ContextMATH.
“w/o” denotes directly solving the scenario with the reasoning model. 
}
\label{tab:two_stage_results}
\end{wraptable}
